Forecasting People Trajectories and Head Poses by Jointly Reasoning on Tracklets and Vislets

In this work, we explore the correlation between people trajectories and their head orientations. We argue that people trajectory and head pose forecasting can be modelled as a joint problem. Recent approaches on trajectory forecasting leverage short-term trajectories (aka tracklets) of pedestrians to predict their future paths. In addition, sociological cues, such as expected destination or pedestrian interaction, are often combined with tracklets. In this paper, we propose MiXing-LSTM (MX-LSTM) to capture the interplay between positions and head orientations (vislets) thanks to a joint unconstrained optimization of full covariance matrices during the LSTM backpropagation. We additionally exploit the head orientations as a proxy for the visual attention, when modeling social interactions. MX-LSTM predicts future pedestrians location and head pose, increasing the standard capabilities of the current approaches on long-term trajectory forecasting. Compared to the state-of-the-art, our approach shows better performances on an extensive set of public benchmarks. MX-LSTM is particularly effective when people move slowly, i.e. the most challenging scenario for all other models. The proposed approach also allows for accurate predictions on a longer time horizon.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/Motivation.tex <==
    %
    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/correlazione.pdf}
		\caption{Motivating the MX-LSTM: a) analysis between the angle discrepancy $\omega$ between head pose and movement, the pedestrain smoothed velocity and the average errors of different approaches on the UCY sequence~\cite{lerner2007crowds}; b) correlation between movement angle $\beta$ and head orientation angle $\alpha$ when the velocity is varying (better in color).}\label{fig:angles}
		\vspace{-10pt}
	\end{center}
    \end{figure*}
    % 

\section{Motivation for the MX-LSTM} \label{sec:dataset}

So far, no quantitative studies focused on how  head pose knowledge impacts on the trajectory forecasting. %Our goal is to show that head pose is helpful for forecasting of the people movements. 
Here, we show a preliminary analysis of the common forecasting datasets with emphasis on the head pose, that motivated the design of the MX-LSTM. 

In particular, we focus on the UCY dataset~\cite{lerner2007crowds}, composed by the Zara01, Zara02, and UCY sequences, which provides the annotations for  the pan angle of the head pose of all the pedestrians.  We also consider the Town Center dataset~\cite{benfold2011stable}, where we manually annotated the head pose, using the same annotation protocol of~\cite{lerner2007crowds}.
%%Marco:why town center is important?
We discover the following facts\footnote{Here is presented the analysis on the UCY sequence, which is similar to what we observed on the other sequences.}:
%\begin{enumerate}
    %\item \vspace{-0.1cm}%
    
    \vspace{.5em}
    \noindent\textbf{1) People often do not watch their steps}. To show this fact(Fig.\ref{fig:explanations}c), for each individual trajectory composed by $T$ frames (omitting the individual indices), we calculate all the $\alpha_t$, $\beta_t$ and $\omega_t$ of Fig.\ref{fig:explanations}c. The $\alpha_t$ is the head pose pan angle with respect to a given reference system; similarly, $\beta_t$ is the angle of motion, and  $\omega_t$ is showing the discrepancy between the two. 
    %%the vislets anchor points $\{\mathbf{a}_t\}_t=1,\dots,T-1$, connected with the corresponding $\{\mathbf{x}_t\}_t=1,\ldots,T-1$, thus forming vectors oriented with the pan angle of the head $\alpha_t$ with respect to a given reference system. Then, we considered the vector modeling the movement between the time steps $t$ and $t+1$ originating at $\mathbf{x}_t$ and leading to $\mathbf{x}_{t+1}$, with angle  $\beta_t$. We compute finally the angle comprised between these two vectors, obtaining the angle $\omega_t$. A graphical explanation is given in Fig.~\ref{fig:explanations}c).
%    The angle $\omega_t$ is showing the discrepancy between the head pan angle and the instantaneous movement of a person.
    For each individual trajectory, we compute the average $\omega = 1/N\sum_{t=1...T}\omega_t$.
    On the multi-y-axis Fig.~\ref{fig:angles}a, we show the $\omega$ value (in degrees) of all the sequences, in an increasing order (blue line and axis). From the figure, we omit those sequences where the speed is below 0.45m/sec.: in those cases the individual is essentially still and the movement vector $\vv{\bm{x_{t+1}-x_{t}}}$ carry few if no meaning, and consequently the angle $\beta_t$ cannot be taken into account. The $\omega$ value ranges from $0.02^{\circ}$ to $72^{\circ}$. We conclude that in ~25\% of the video sequences the misalignment between the head pose and the step direction is larger than
 $20^{\circ}$.
    
    %\item \vspace{-0.1cm} 
    \vspace{.5em}
    \noindent\textbf{2) Head pose and movements are (statistically) correlated};
    On the same figure, we report the velocity curve (black solid line and axis), where each y-point  gives the average speed of the $i-th$ ordered trajectory on the x-axis~\footnote{For the sake of readability, the curve has been smoothed with moving average filter of size 10.}.   As it shows, there is a relation of inverse proportionality between the $\omega$ and the pedestrian speed: the alignment between the head towards the direction of movement is higher when the speed is higher; when the person slows down the head pose is dramatically misaligned. The relation is statistically significant: we consider the Pearson circular correlation coefficient~\cite{jammalamadaka2001topics} between the angles $\alpha_{t}$ and $\beta_t$, computed over all the frames of the sequences considered for that figure. On the whole data, the correlation is 0.83 (p-value$<0.01$).
    %, indicating a linear relation between the two quantities. 
    We also investigate how the correlation changes with the speed: Fig.~\ref{fig:angles}b shows the correlation values against velocity, computed by pooling the $\alpha_{t}$ and $\beta_t$ angles around a certain velocity value; in particular, each correlation value at velocity $\tau$ has been computed by considering all of the samples in the range $[\tau-0.01R, \tau +0.01R]$, where $R$ is the whole velocity range. All the reported values have statistical significance (p-value$<0.01$). The plot shows clearly that the correlation is lower at low velocities, where the discrepancy between the $\alpha_t$ and $\beta_t$ angles is in general higher.  
    %
    The challenge here is to investigate whether this discrepancy can be learned by the MX-LSTM to improve the forecasting. More intriguingly, MX-LSTM should learn how these relations evolve in time, which has not been investigated yet, since the analysis done so far consider each time instant as independent from each other.  
    
    %\item \vspace{-0.1cm}
    \vspace{.5em}
    \noindent\textbf{3) Forecasting errors are in general higher when the speed of the pedestrian is lower}; In Fig.~\ref{fig:angles} are reported the Mean Average Displacement (MAD) error~\cite{pellegrini2009iccv} (red line and axis) of the following approaches: SF~\cite{yamaguchi2011cvpr}, LTA~\cite{trautman2010iros}, vanilla LSTM and Social LSTM~\cite{alahi2016cvpr}, together with our MX-LSTM approach.  In general, lower velocities bring to higher errors, since when people are walking very slowly their behavior become less predictable, due to physical reasons (less inertia) but also behavioral (people walking slowly are usually involved into other activities, like talking with other people, looking around). On the contrary, it is shown here that  MX-LSTM is performing well  even at lower velocities, reaching errors very close to zero with static people (more details in Sec.\ref{sec:experiments}). 



%The modeling of the social context may help (like the Social LSTM~\cite{alahi2016cvpr} case, see the additional material), but still in this case, prediction errors when people are semi static or slow are of the same magnitude of the ones when people is moving fast.  
%\end{enumerate}
%Similar observations hold for the other datasets too, which will be reported in the additional material. \\
%\vspace{0.5em}
Summarizing, head pose is correlated with the movement, especially when people move fast. When people move slow, the correlation is weaker but significant, the prediction errors are larger, and the head pose is drastically misaligned with the movement. These facts justify and motivate our objective with the MX-LSTM, to capture the head pose information jointly with the movement and use it for a better forecasting.
%
%--------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------
%


==> sections/experiment_irtiza_backup.tex <==
\vspace{-0.1cm} \section{Experiments}\label{sec:experiments}


We present here both quantitative and qualitative experiments.
Quantitative results validate the proposed MX-LSTM model, setting the new state-of-the-art for trajectory forecasting; results are also provided for an ablation study showing the importance of the different parts of the MX-LSTM. Furthermore, whether ground truth (GT) head pose information can be substituted by more accessible proxies, like step directions or simple head pose estimations (from a detector). We also present in detail the analysis of our approach with respect to different horizon intervals. We also discuss how MX-LSTM performs in long term forecasting. Additionally, we illustrate how head pose plays a pivotal role for the long term forecasting. Finally, we present the very first results on head pose forecasting. Qualitative results unveil the interplay between tracklets and vislets that the MX-LSTM has learnt. 

%% introduction
% The experiments are quantitative and qualitative. The former evaluate MX-LSTM and some variants on 4 datasets (the 3 UCY sequences Zara01, Zara02 and UCY~\cite{lerner2007crowds}, and the Town Centre dataset~\cite{benfold2011stable}); all the sequences have ground truth head poses, while on the Town Centre we manually added ground truth head poses and head poses estimated by~\cite{}. In all the cases,  the head poses are expressed as pan angles over the 360 circle. Comparative approaches are: Social Force model (SF)~\cite{}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}; in addition we use a vanilla LSTM model as baseline, removing the social pooling from the S-LSTM.
%\vspace{-0.1cm}



\subsection{Evaluation Metrics}\label{sec:metrics}

In all the cases,  the head poses are expressed as pan angles over the 360$^\circ$. Trajectory forecasting methods are qunatitively analyzed by Mean Average Displacement (MAD) error, average euclidean distance between predicted point and ground truth point. Furthermore, we also evaluate Final Average Displacement error as a measure of quality which is essentially euclidean distance between the last predicted point and corresponding ground truth point.   

\subsection{Datasets}\label{sec:datasets}
\myparagraph{UCY dataset.}
UCY dataset~\cite{lerner2007crowds} composed of three sequences namely Zara01, Zara02, and UCY.
All the sequences have ground truth head poses.

\myparagraph{TownCenter.}
we manually annotated ground truth head poses on TownCenter. We make public all the annotations done on TownCenter

\subsection{Implementation Details}\label{sec:impl}
For training MX-LSTM and the ablation study models, we use a learning rate of 0.005 along with the RMS-prop optimizer. We set the embedding dimension for spatial coordinates
and vislets to 64 and the hidden state dimension is D = 128.The grid for the social pooling (Eq.~\eqref{eq:social}) has $N_o\times N_o$ cells with $N_o=32$. The view frustum aperture angle has been cross-validated on the training partition of the TownCenter and kept fixed for the remaining trials ($\gamma=40^{\circ}$), while the depth $d$ is simply bounded by the social pooling grid. The MX-LSTM was train on a single GPU with Tensorflow~\cite{abadi2016tensorflow} implementation. 


\subsection{Ablation Study}\label{sec:ablation}
Aside with the models in the literature, we investigate three variations of the MX-LSTM to capture the net contributions of the different parts that characterize our approach.

\noindent\textbf{Block-Diagonal MX-LSTM (BD-MX-LSTM)}: it serves to highlight the importance of estimating full covariances to understand the interplay between tracklets and vislets.  
%
%enforcing the LSTM to jointly studying the separated information streams, tracklets and vislets, through the full covariance. Essentially, instead of learning the $4\times4$ full $\mathbf{\Sigma}$, 
%
Essentially, the approach estimates two bidimensional covariances\footnote{The $2\times2$ covariance is estimated employing two variances $\sigma_1, \sigma_2$ and a correlation terms $\rho$ as presented in \cite{graves2013generating} Eq.(24) and (25).} $\mathbf{\Sigma}_x$ and $\mathbf{\Sigma}_a$ for the trajectory and the vislet modeling respectively, without capturing the cross-stream covariances.

% \emph{The equations that differ w.r.t. MX-LSTM will be given as supplemental material.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
are Eq. (\ref{eq:LLog}) and (\ref{eq:params}), which become, respectively, 
\begin{eqnarray}
L^i(\mathbf{W}_{x},\mathbf{W}_{a},\mathbf{W}_H,\mathbf{W}_{\text{LSTM}},\mathbf{W}_{o}) &=&\nonumber\\  -\sum_{T_{obs}+1}^{T_{pred}}log\left( P([\mathbf{x}^{(i)}_t]^T|\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t \right)+\!\!\\\nonumber
log\left(P([\mathbf{a}^{(i)}_t]^T|\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t\right)
\end{eqnarray}
where $\bo{\mu}^{(x,i)}_t=[{}_x\mu^{(x,i)}_t,{}_y\mu^{(x,i)}_t]$ and the same apply for the variance vector;
\begin{equation}
[\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t,\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t]^T \!=\! \mathbf{W}_o \mathbf{h}^{(i)}_{t-1}\label{eq:params}
\end{equation}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{NoFrustum MX-LSTM}: this variation of the MX-LSTM uses social pooling as in~\cite{alahi2016cvpr}, in which the interest area where people hidden states $\{\mathbf{h}^{j}_t\}$ are pooled into the social tensor  all around the individual. In other words, no frustum selecting the people that have to be considered is used here.

\noindent\textbf{Individual MX-LSTM}: In this case, no social pooling is taken into account, therefore the embedding operation of Eq.~(\ref{eq:pooling}) is absent, and the weight matrix $\mathbf{W}_H$ vanishes. In practice, this variant learns independent models for each person, each one considering the tracklet and vislet points.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Error metric (MAD). 12, 14…32 corresponds to horizon intervals for prediction. Observation interval is kept constant (8 frames). Smaller Observation Interval, H=12. larger Observation=16 Interval larger prediction interval.}
% \label{table:table1}
% \resizebox{.999\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|}
% \cline{1-8} \cline{10-13} \cline{15-19}
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{\underline{H = 12}} & \textbf{H = 16} & \textbf{H = 20} & \textbf{H = 24} & \textbf{H = 28} & \textbf{H = 32} &  & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} &  & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.90            & 1.21            & 1.70            & 2.30            & 3.07            & 4.11            &  & 1.62             & 0.90             & 0.90             & 0.90              &  & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.72            & 1.05            & 1.44            & 1.85            & 2.47            & 3.14            &  & 1.43             & 0.79             & 0.72             & 0.60              &  & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.68            & 1.00            & 1.43            & 1.94            & 2.35            & 2.85            &  & \textbf{0.89}             & 0.69             & 0.68             & 0.68              &  & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.59}   & \textbf{0.87}   & \textbf{1.21}   & \textbf{1.55}   & \textbf{1.92}   & \textbf{2.40}   &  & 0.96    & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     &  & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 1.09            & 1.62            & 2.19            & 2.75            & 3.31            & 3.86            &  & 1.65             & 1.17             & 1.09             & 0.99              &  & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.63            & 1.09            & 1.43            & 1.83            & 2.25            & 2.67            &  & 1.35             & 0.84             & 0.63             & 0.62              &  & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.63            & 0.90            & 1.24            & 1.59            & 2.00            & 2.41            &  & 1.13             & 0.74             & 0.63             & 0.63              &  & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.35}   & \textbf{0.53}   & \textbf{0.71}   & \textbf{0.90}   & \textbf{1.16}   & \textbf{1.40}   &  & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     &  & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.67            & 0.90            & 1.19            & 1.52            & 1.87            & 2.24            &  & 0.82             & 0.65             & 0.67             & 0.63              &  & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.53            & 0.77            & 1.01            & 1.27            & 1.53            & 1.83            &  & 0.88             & 0.59             & 0.53             & 0.52              &  & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.62            & 0.90            & 1.08            & 1.36            & 1.66            & 1.99            &  & 0.71             & 0.63             & 0.62             & 0.60              &  & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.49}   & \textbf{0.70}   & \textbf{0.95}   & \textbf{1.22}   & \textbf{1.50}   & \textbf{1.80}   &  & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     &  & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Error metric (MAD). 12, 14…32 corresponds to horizon intervals for prediction. Observation interval is kept constant (8 frames). Smaller Observation Interval, H=12. larger Observation=16 Interval larger prediction interval.}
% \label{table:table1}
% \resizebox{.999\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c!{\vrule width2pt}c|c|c|c!{\vrule width2pt}c|c|c|c|c|}
% \hline
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{\underline{H = 12}} & \textbf{H = 16} & \textbf{H = 20} & \textbf{H = 24} & \textbf{H = 28} & \textbf{H = 32} & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \hline
% \multirow{4}{*}{\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.90            & 1.21            & 1.70            & 2.30            & 3.07            & 4.11            & 1.62             & 0.90             & 0.90             & 0.90              & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.72            & 1.05            & 1.44            & 1.85            & 2.47            & 3.14            & 1.43             & 0.79             & 0.72             & 0.60              & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.68            & 1.00            & 1.43            & 1.94            & 2.35            & 2.85            & 0.89             & 0.69             & 0.68             & 0.68              & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.59}   & \textbf{0.87}   & \textbf{1.21}   & \textbf{1.55}   & \textbf{1.92}   & \textbf{2.40}   & \textbf{0.96}    & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \hline
% \multirow{4}{*}{\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 1.09            & 1.62            & 2.19            & 2.75            & 3.31            & 3.86            & 1.65             & 1.17             & 1.09             & 0.99              & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.63            & 1.09            & 1.43            & 1.83            & 2.25            & 2.67            & 1.35             & 0.84             & 0.63             & 0.62              & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.63            & 0.90            & 1.24            & 1.59            & 2.00            & 2.41            & 1.13             & 0.74             & 0.63             & 0.63              & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.35}   & \textbf{0.53}   & \textbf{0.71}   & \textbf{0.90}   & \textbf{1.16}   & \textbf{1.40}   & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \hline
% \multirow{4}{*}{\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.67            & 0.90            & 1.19            & 1.52            & 1.87            & 2.24            & 0.82             & 0.65             & 0.67             & 0.63              & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.53            & 0.77            & 1.01            & 1.27            & 1.53            & 1.83            & 0.88             & 0.59             & 0.53             & 0.52              & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.62            & 0.90            & 1.08            & 1.36            & 1.66            & 1.99            & 0.71             & 0.63             & 0.62             & 0.60              & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.49}   & \textbf{0.70}   & \textbf{0.95}   & \textbf{1.22}   & \textbf{1.50}   & \textbf{1.80}   & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \hline
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\renewcommand{\arraystretch}{2}
\begin{table}[!htb]
\centering
\caption{Error metric (MAD). 12, 14…32 corresponds to horizon intervals for prediction. Observation interval is kept constant (8 frames).}
\label{table:table1Ab}
\resizebox{.999\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
{\textbf{Dataset}} & {\textbf{Method}}                                                 & {\textbf{\underline{H = 12}}} & {\textbf{H = 16}} & {\textbf{H = 20}} & {\textbf{H = 24}} & {\textbf{H = 28}} & {\textbf{H = 32}} \\ \cline{1-8} 
                                  \multirow{4}{*}{\vspace{-35pt}\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 0.90                & 1.21                & 1.70                & 2.30                & 30.7                & 4.11                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.72                & 1.05                & 1.44                & 1.85                & 2.47                & 3.14                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.68                & 1.00                & 1.43                & 1.94                & 2.35                & 2.85                \\ \cline{2-8} 
                                  & \textbf{MX-LSTM}                                                     & \textbf{0.59}       & \textbf{0.87}       & \textbf{1.21}       & \textbf{1.55}       & \textbf{1.92}       & \textbf{2.40}       \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.09                & 1.62                & 2.19                & 2.75                & 3.31                & 3.86                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.63                & 1.09                & 1.43                & 1.83                & 2.25                & 2.67                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.63                & 0.90                & 1.24                & 1.59                & 2.00                & 2.41                \\ \cline{2-8} 
                                  & \textbf{MX-LSTM}                                                     & \textbf{0.35}       & \textbf{0.53}       & \textbf{0.71}       & \textbf{0.90}       & \textbf{1.16}       & \textbf{1.40}       \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 0.67                & 0.90                & 1.19                & 1.52                & 1.87                & 2.24                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.53                & 0.77                & 1.01                & 1.27                & 1.53                & 1.83                \\ \cline{2-8} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.62                & 0.90                & 1.08                & 1.36                & 1.66                & 1.99                \\ \cline{2-8} 
                                  & \textbf{MX-LSTM}                                                     & \textbf{0.49}       & \textbf{0.70}       & \textbf{0.95}       & \textbf{1.22}       & \textbf{1.50}       & \textbf{1.80}       \\ \hline
\end{tabular}}
\end{table}
\renewcommand{\arraystretch}{1}

\renewcommand{\arraystretch}{2}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\caption{Smaller Observation Interval, H=12.}
\label{table:table2Ab}
\resizebox{.999\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.62             & 0.90             & 0.90             & 0.90              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 1.43             & 0.79             & 0.72             & 0.60              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & \textbf{0.89}    & 0.69             & 0.68             & 0.68              \\ \cline{2-6} 
                                  & \textbf{MX-LSTM}                                                      & 0.96             & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.65             & 1.17             & 1.09             & 0.99              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 1.35             & 0.84             & 0.63             & 0.62              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 1.13             & 0.74             & 0.63             & 0.63              \\ \cline{2-6} 
                                  & \textbf{MX-LSTM}                                                      & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 0.82             & 0.65             & 0.67             & 0.63              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.88             & 0.59             & 0.53             & 0.52              \\ \cline{2-6} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.71             & 0.63             & 0.62             & 0.60              \\ \cline{2-6} 
                                  & \textbf{MX-LSTM}                                                      & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     \\ \hline
\end{tabular}}
\end{table}
\renewcommand{\arraystretch}{1}

\renewcommand{\arraystretch}{2}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\caption{larger Observation=16 Interval larger prediction interval.}
\label{table:table3Ab}
\resizebox{.999\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-7} 
                                  & \textbf{MX-LSTM}                                                      & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-7} 
                                  & \textbf{MX-LSTM}                                                      & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \hline
\multirow{4}{*}{\vspace{-35pt}\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-7} 
                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-7} 
                                  & \textbf{MX-LSTM}                                                      & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \hline
\end{tabular}}
\end{table}
\renewcommand{\arraystretch}{1}

\vspace{1em}
Table~\ref{tab:res-oracle}, last three columns, reports numerical results for all the MX-LSTM simplifications on all the datasets. The main facts that emerge are: 1) the highest variations are with the Zara02 sequence, where MX-LSTM doubles the performances of the worst approach (Individual MX-LSTM); 2) the worst performing is in general Individual MX-LSTM, showing that social reasoning is indeed necessary; 3) social reasoning is systematically improved with the help of the vislet-based view-frustum; 4) full covariance estimation has a role in pushing down the error which is already small with the adoption of vislets.  

Summarizing the results so far, having vislets as input allows to definitely increase the trajectory forecasting performance, even if vislets are estimated with noise. Vislets should be used to understand social interactions with social pooling, by building a view frustum that tells which are the people currently observed by each individual. All of these features are done efficiently by the MX-LSTM: in fact the training time is the same with having an LSTM with social pooling.


%Again, although the complete method always outperforms all the competitors, the highest improvement is on the TownCentre sequence. In our opinion this is due to the different level of complexity in the data, indeed most of the trajectories in UCY sequences are relatively linear, with poor social interactions, while in TownCentre there are many interactions like forming and splitting groups, and crossing trajectories.
%For the same reason, this is also the only dataset where the introduction of the view frustum in the pooling of social interactions gives the highest benefits. In all the sequences instead, %decoupling the covariance matrix into a block diagonal matrix 
%neglecting the interplay of position and gaze (Unmixed LSTM) leads to a sensitive increase in the prediction error; this proves the tight relation between the head orientation and the motion of an individual.

\subsubsection{Head Pose Forecasting}\vspace{-0.1cm}
As done with trajectories, we are also providing a forecast of the head pose of each individual at each frame which is a distinctive attribute of our method.   We evaluate the performances of this estimation in terms of mean angular error $e_{\alpha}$, which is the mean absolute difference between the estimated pose (angle $\alpha_{t,\cdot}$ in Fig.~\ref{fig:explanations}c) and the annotated GT.
%is equal to the pose plausibility error, with $\alpha_{t,\cdot}$ instead of $\omega_{t,\cdot}$. It tells how much the direction in which is looking an individual at a particular instant is different wrt the real direction, independently on where the individual has been predicted to be located. Having a low $e_{\alpha}$ means that in general we are guessing correctly the direction of interest, especially in coincidence with a low MAD, as it is in general in our experiments.   

% \begin{table}[t!]
%   \centering
%   \caption{Pose plausibility error ($e_{\text{pp}}$) and angular error ($e_{\alpha}$) for the MX-LSTM model on all the datasets.}
%   \label{tab:res-angle}
%   \begin{tabular}{|l|*{2}{C{.1\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     TownCentre &  23.30  &  26.48  \\
%     \hline
%   \end{tabular}
% \end{table}

\renewcommand{\arraystretch}{2}
\begin{table}[t!]
  \centering
  \small
  \caption{Mean angular error (in degrees) for the state-of-the-art head pose estimator~\cite{lee2015fast}, and the MX-LSTM model fed with GT annotations and estimated values (MX-LSTM-HPE).}
  \label{tab:res-angle}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{|l|c|c|c|c|}
    \hline
    Metric                &  Zara01  &  Zara02  &   UCY   &  Town Centre \\
    \hline
    HPE~\cite{lee2015fast} & 14.29   &   20.02  &  19.90 &   25.08    \\   
    \hline
    MX-LSTM               &  12.98   &   20.55  &  21.36  &   26.48    \\
    \hline
    MX-LSTM-HPE  &  17.69   &   21.92  &  24.37  &   28.55  \\
    \hline
  \end{tabular}
  }
\end{table}
\renewcommand{\arraystretch}{1}





% \begin{table}[t!]
%   \centering
%   \begin{minipage}[t]{.39\columnwidth}
%     \centering
%     \caption{Head pose estimation errors for MX-LSTM on all the datasets (in degrees).}
%     \label{tab:res-angle}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{|l|*{2}{C{.25\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     Town Centre &  23.30  &  26.48  \\
%     \hline
%     \end{tabular}
%     }
%   \end{minipage}
%   \hspace{.02\linewidth}
%   \begin{minipage}[t]{.57\columnwidth}
%     \centering
%     \caption{Boh}
%     \label{fig:angle}
%     \includegraphics[width=\linewidth]{figure/supercool.pdf}
%   \end{minipage}
% \end{table}



Table~\ref{tab:res-angle} shows numerical results of the static head pose estimator~\cite{lee2015fast} (HPE), the MX-LSTM using GT head poses, and the MX-LSTM fed with the output of HPE during the observation period (MX-LSTM-HPE).
In all the cases our forecast output is comparable with the one of HPE, but in our case we do not use appearance cues -- i.e. we do not look at the images at all.
In case of Zara01, the MX-LSTM is even better that the static prediction showing the forecasting power of our model. In our opinion this is due to the fact that in this sequence trajectories are mostly very linear and fast, and heads are mostly aligned with the direction of motion. When we provide estimations to the MX-LSTM model during the observation period, angular error increases, as expected. Despite this, the error is surprisingly limited.
%The low error achieved in Zara01 is probably related to the fact that this sequence is dominated people moving linearly and fast, thus the head orientation is usually aligned with the trajectory and the model can learn this behavior very easily.
%Zara02: more complicate, people are standing more in between of people moving fast (right Irtiza?) so big variety of disalignments, and you have the biggest errors
%Zara02 is a more challenging sequence, since there is a high number of standing group formations in the middle of the scene; these trajectories are very noisy, and as a consequence $e_{\text{pp}}$ increase.
%UCY: still group formations, but they are moving, so less disalignment and noise, numbers are in accord with this (Irtiza agree?)
%In UCY, the grouping formations are still present, but in this case they are moving, so noise is reduced and thus the disalignement between trajectory and head pose.

\input{sections/table_stateoftheart_comparison}

\subsubsection{Horizon Effect}\label{sec:horizon}
% \todo{ Explain the bullet points and place all the relevant tables
% \begin{itemize}
%     \item We show that MX-LSTM is also more accurate in long term forecasting;
%     %the head pose, also given by a normal head pose estimator;\vspace{-5pt}
%     \item we illustrate that social LSTM degrades as we increase the prediction interval
%     \item We motivate that even with fewer observation interval the injection of head pose provides useful information in long term forecasting. 
%     \item We present ranking order remains same in all experiment.
% \end{itemize}
% }

In order to understand, how MX-LSTM performs for longer time interval we conducted an experimental evaluation where we increment the prediction interval from 12 to 32 frames with the step size of 4, keeping the observation interval fixed at 8 frames. We use MAD to report the error. As shown in table~\ref{table:table1Ab}, MX-LSTM is well capable of handling longer time horizons. MX-LSTM outperforms all other approaches on all prediction interval, showing the robustness of MX-LSTM. Furthermore, it can also be argued that head pose, especially in long term forecasting serves even more crucially. The ranking is preserved (MX-LSTM) having the lowest error.  

Similarly, in table~\ref{table:table2Ab}, we wanted to see what observation interval is sufficient for an LSTM based model to learn the general shape of the trajectory. Therefore, we kept the prediction interval fixed at 12 frames and varied the observation interval form 1 to 16 frames with the step size of 4 frames. As it can be seen 1 frame is basically not enough for any approach, and all approaches gives inferior performances, though MX-LSTM except for zara01, performs still better than other approaches. Interestingly, a rapid drop in error of roughly ~30 \% can already be seen just by observing 4 frames instead of 1. Furthermore, it can been observed that 8 frames are enough for the approaches to learn the over shape of the trajectory in order to predict for the next 12 frames, as the error drop from observing 8 frames to 16 frames is below 1\%.

Finally, in order to understand in more depth, long term forecasting. We kept the observation interval constant at 16 frames. Table~\ref{table:table3Ab}, further validates the fact that 8 frames are sufficient for the LSTM approach to learn the representation of the trajectory. MX-LSTM, still the best performer but the error drop from observing 8 to observing 16 frames is negligible in long term forecatsing as well. This affect also illustrates about the capacity of the LSTM based approach. At 8 frames, the performance already starts to saturate, therefore adding more information does not bring any new meaningful information to learn. This can bee seen as the performance bottle neck of all LSTM based approaches.   

\subsubsection{Substitute for Head Pose}\vspace{-0.1cm}
In this experiment we mainly focused on the head pose, wondering whether ground truth (GT) head pose information can be substituted by more accessible proxies, like step directions or simple head pose estimations. Quantitatively,
we implemented a Pace-MX-LSTM, which uses ground truth step directions instead of the head pose. Looking at the Table~\ref{table:step} illustrates the fact that Having the step direction instead of the head pose represents a downgrade for MX-LSTM, since positional data are already contained in the tracklet and the step direction can be extracted from the previous two positions. Therefore, Pace-MX-LSTM gives consistently worse results. Additionally, We implemented the MX-LSTM-HPE-Train and Test,
where the head pose training data is given by a detector~\cite{hasan2017tiny}. Performances (see ~\ref{table:step}) are obviously worse than MX-LSTM-HPE (where only the test sequences consist of
head pose estimations), especially on Zara02, where conversational groups make the head pose estimation noisy due to the many partial occlusions. Still MX-LSTM-HPE-Train
and Test performs comparable to the prior state-of-the-art.



\subsection{Comparison with Recent Approaches}\label{sec:sota}

% \subsection{Quantitative results}

%% Oracle experiments

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets.}
%   \label{tab:res-oracle}
%   \begin{tabular}{|c|l|*{6}{C{.093\textwidth}|}}
%     \hline
%     Metric & Dataset    &  SF~\cite{yamaguchi2011cvpr}  &  LTA~\cite{pellegrini2009iccv}   &  Vanilla LSTM~\cite{alahi2016cvpr}  & Social LSTM~\cite{alahi2016cvpr} & MX-LSTM  & {\it MX-LSTM (real HPE)} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara01 & 2.88 & 2.74 & 0.90 & 0.68 & {\bf 0.59} & {\it 0.66} \\
%     \cline{2-8}
%     & Zara02    & 2.32 & 2.23 & 1.09 & 0.63 & {\bf 0.35} & {\it 0.37} \\
%     \cline{2-8}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & {\bf 0.49} & {\it 0.55} \\
%     \cline{2-8}
%     & TownCentre &9.35 &9.14   & 4.62 & 1.96 & {\bf 1.15} & {\it 1.21} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara01 & 5.55 & 5.55 & 1.85 & 1.53 & {\bf 1.31} & {\it 1.43} \\
%     \cline{2-8}
%     & Zara02    &  4.35 &  4.35 & 2.15 & 1.43 & {\bf 0.79} & {\it 0.82} \\
%     \cline{2-8}
%     & UCY        &  4.62 &  4.66 & 1.39 & 1.40 & {\bf 1.12} & {\it1.20 } \\
%     \cline{2-8}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & {\bf 2.30} & {\it 2.38} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

%\subsection{Quantitative results}\label{sec:quantitative}\vspace{-0.1cm}
We compare the performance of our model with the following related approaches: Social Force model (SF)~\cite{yamaguchi2011cvpr}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, Vanilla LSTM, Social LSTM (S-LSTM)~\cite{alahi2016cvpr} and Social GAN~\cite{SocialGAN18}. The evaluation protocol is the same as with~\cite{pellegrini2009iccv}, where the algorithm receives 8 ``observation'' ground truth (GT) frames of a trajectory to predict the following 12 ones.

For the three UCY sequences three models have been trained. For each model, we use two sequences for training and then we test on the third one. For Town Centre dataset, the model has been trained and tested on the provided data splits.

Regarding the model parameters, the social pooling grid (Eq.~\eqref{eq:social}) has $N_o\times N_o$ cells with $N_o=32$. The view frustum aperture angle has been cross-validated on the training partition of the Town Center and kept fixed for the remaining trials ($\gamma=40^{\circ}$), while the depth $d$ is simply bounded by the social pooling grid. 

The trajectory prediction performance is evaluated based on the Mean Average Displacement (MAD) error (euclidean distance between predicted and GT points, averaged over the sequence) and the Final Average Displacement (FAD) error (distance between the last predicted point and the corresponding GT point)~\cite{pellegrini2009iccv}.

The results are reported in Tab.~\ref{tab:res-oracle}. The MX-LSTM outperforms the state-of-the-art methods in every single sequence and with both  metrics, with an average improvement of 23.3\%. The highest relative gain is achieved in UCY and Town Centre datasets, where complex non-linear paths are mostly caused by standing conversational groups and people that walk close to them, avoiding collisions. People slowing down and looking at the window shops pose another challenge. As shown in Fig.~\ref{fig:angles}, slow moving and interacting pedestrians cause troubles to the competing methods, while MX-LSTM clearly overcomes such shortcomings denoting a better model. Note that the Social GAN~\cite{SocialGAN18} is the only method that uses ground-truth trajectories during prediction interval. The Social GAN~\cite{SocialGAN18} model predicts 20 trajectories and uses the L2 distance with the ground truth trajectory to pick the best one, which brings an intrinsic contradiction. This advantage is visible in the most linear dataset Zara01, where Social GAn~\cite{SocialGAN18} performs better than the proposed approach. Qualitative evaluation follows in Sec.~\ref{sec:qualitative}. 

The evaluated method rely on different input data: SF and LTA require the destination point of each individual, while SF requires social groups annotations. MX-LSTM requires the head pose of each individual for the first 8 frames that can be estimated by a head pose estimator. This motivates our next experiment: we automatically estimate the head bounding box given the feet positions on the floor plane, assuming an average person being $1.80$m tall. Then, we apply the head pose estimator of~\cite{lee2015fast} that provides continuous angles. They can be used as input to our approach, noted as ``MX-LSTM-HPE''.   

As shown by the scores in Tab.~\ref{tab:res-oracle}, MX-LSTM-HPE does not suffer from small errors in the input head pose, with an average drop in performances of only 5\%. In addition, MX-LSTM-HPE outperforms all related methods on all datasets, even with the noisy estimated head pose information.

How accurate should the head pose estimation be, for the MX-LSTM-HPE to have convincing performances, for example outperforming the Social LSTM? We answer this question by corrupting the true head pose estimate with additive Gaussian noise$\sim\mathcal{N}(\alpha_t,\hat{\sigma})$, where $\alpha_t$ is the correct head pose and $\hat{\sigma}$ the standard deviation. MX-LSTM-HPE outperforms social-LSTM up to a noise of $\hat{\sigma}=24^{\circ}$.


%% Ablation study
%\subsubsection*{Ablation study}

%% ----------------------------------
%%  two columns
%% ----------------------------------
% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on all the datasets for three variations of the proposed MX-LSTM method. The last column reports the results of the proposed model to ease the comparison.}
%   \label{tab:res-variations}
%   \begin{tabular}{|c|l|*{4}{C{.095\textwidth}|}}
%     \hline
%     Metric & Dataset    &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara01 & 0.63 & 0.63 & 0.60 & {\bf 0.59} \\
%     \cline{2-6}
%     & Zara02    & 0.72 & 0.36 & 0.41 & {\bf 0.35} \\
%     \cline{2-6}
%     & UCY        & 0.53 & 0.51 & 0.54 & {\bf 0.49} \\
%     \cline{2-6}
%     & TownCentre & 2.09 & 1.70 & 1.40 & {\bf 1.15} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 2.18} & {\it 1.70} & {\it 1.44} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara01 & 1.37 & 1.40 & 1.51 & {\bf 1.31} \\
%     \cline{2-6}
%     & Zara02    & 1.56 & 0.84 & 1.00 & {\bf 0.79} \\
%     \cline{2-6}
%     & UCY        & 1.16 & 1.15 & 1.23 & {\bf 1.12} \\
%     \cline{2-6}
%     & TownCentre & 4.00 & 3.40 & 2.90 & {\bf 2.3} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 4.20} & {\it 3.40} & {\it 3.0} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

%% ----------------------------------
%%  single column
%% ----------------------------------
% \begin{table}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on all the datasets for three variations of the proposed MX-LSTM method. The last column reports the results of the proposed model to ease the comparison.}
%   \label{tab:res-variations}
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{|c|l|*{4}{C{.093\textwidth}|}}
%     \hline
%     Metric & Dataset    &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{4}{*}{\centering MAD} & Zara01 & 0.63 & 0.63 & 0.60 & {\bf 0.59} \\
%     \cline{2-6}
%     & Zara02    & 0.72 & 0.36 & 0.41 & {\bf 0.35} \\
%     \cline{2-6}
%     & UCY        & 0.53 & 0.51 & 0.54 & {\bf 0.49} \\
%     \cline{2-6}
%     & TownCentre & 2.09 & 1.70 & 1.40 & {\bf 1.15} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 2.18} & {\it 1.70} & {\it 1.44} & {\it 1.21} \\
%     \hline \hline
%     \multirow{4}{*}{\centering FAD} & Zara01 & 1.37 & 1.40 & 1.51 & {\bf 1.31} \\
%     \cline{2-6}
%     & Zara02    & 1.56 & 0.84 & 1.00 & {\bf 0.79} \\
%     \cline{2-6}
%     & UCY        & 1.16 & 1.15 & 1.23 & {\bf 1.12} \\
%     \cline{2-6}
%     & TownCentre & 4.00 & 3.40 & 2.90 & {\bf 2.3} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 4.20} & {\it 3.40} & {\it 3.0} & {\it 2.38} \\
%     \hline
%   \end{tabular}
%   }
% \end{table}
%\vspace{-0.2cm}
%\subsubsection{Ablation study}\label{sec:ablation}


%\subsection*{Head pose prediction}
%\vspace{1em}
% Since MX-LSTM predicts the head pose too, we should have a quality measure on it. We propose two types of errors: the \emph{pose plausibility error} $e_{\text{pp}}$, which measures how much the head pose is compatible with the predicted trajectory, considering that we are not contortionists, and the \emph{angular error} $e_{\alpha}$, which evaluates the error of the predicted head pose angle with respect to the ground truth one.

% The $e_{\text{pp}}$ is computed in the following way (see Fig.~\ref{fig:explanations} for the notation): let $\Delta_\omega(t) = |\omega_{t,real}-\omega_{t,pred}|$, where $\omega_t$ is the angle between the vislet and the tracklets at time $t$. Then $e_{\text{pp}}=\min \left( \Delta_\omega(t),180 -\Delta_\omega(t)\right)$. Having a low $e_{\text{pp}}$ means to predict head poses that are anatomically plausible with the predicted movement.
\vspace{-0.2cm}

\subsection{Qualitative Results}\label{sec:qualitative}
\vspace{-0.1cm}
    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/Qualitative8_theo.png}
		\caption{Qualitative results: a) MX-LSTM  b) Ablation qualitative study on Individual MX-LSTM (better in color).}\label{fig:Qualitative}
		\vspace{-15pt}
	\end{center}
    \end{figure*}

Fig.~\ref{fig:Qualitative} shows  qualitative results on the Zara02 dataset, which has been shown to be the most complex scenario in the quantitative experiments
%\footnote{Please check supplemental material for further results.}. 
%
Fig.~\ref{fig:Qualitative}a presents MX-LSTM results: a group scenario is taken into account, with the attention focused on the girl in the bottom-left corner. In the left column, the green ground-truth prediction vislets show that the girl is conversing with the group members, with a movement close to zero and the pan head angle which oscillates. In magenta, the behavior of the S-LSTM, predicting erroneously the girl leaving the group. This error confirms the problem of competing methods in forecasting the motion of people slowly moving or static as discussed in Sec.\ref{sec:dataset}, and further confirmed by the results of the quantitative experiments. %, which show that when people are moving slowly or are static, forecasting error are in general dramatic.
In the central column, the observation sequence given to the MX-LSTM is shown in orange (almost static with oscillating vislets). The related prediction (in yellow) shows oscillating vislets, and almost no movement, confirming that the MX-LSTM has learnt this particular social behavior. If we provide to MX-LSTM an artificial observation sequence with the annotated positions (real trajectory) but vislets oriented toward west  (third column, orange arrows), where no people are present, the MX-LSTM predicts a trajectory departing from the group (cyan trajectory and arrows).


The two rows of Fig.~\ref{fig:Qualitative}b) analyze the Individual MX-LSTM, in which no social pooling is taken into account. Therefore, here each pedestrian is not influenced by the surrounding people, and the relationship between the tracklets and the vislets in the prediction can be observed without any confounding factor. 
%These figures show different types of trajectories, each one equipped with its own vislets, here represented by the tip of the arrows: the blue one, which represents the routing input sequence given to the MX-LSTM. The green one is the ground-truth that has to be predicted. The yellow one is the prediction by MX-LSTM. The magenta one (left column) has been obtained by enforcing the vislets of the routing input sequence to point north (w.r.t. the image plane). The black one (center column) is the same as the magenta one, but pointing north. The red one (right column) has randomly placed vislets. The rationale of these last three types of sequences is to evaluate whether a different head pose behavior could trigger a diverse trajectory prediction. 
Fig.~\ref{fig:Qualitative}b) first row shows three situations in which the vislets of the observation sequence are artificially made pointing north (orange arrows), resulting not aligned with the trajectory. In this case the Individual MX-LSTM predicts a decelerating trajectory drifting toward north (magenta trajectory and vislets), especially in the second and third pictures.  If the observation has the legit vislets (green arrows, barely visible since they are aligned with the trajectory), the resulting trajectory (yellow trajectory and vislets) has a different behavior, closer to the GT (green trajectory and vislets). The second row is similar, with the observation vislets made pointing to south. The prediction with the modified vislets is in black. The only difference is in the bottom left picture: here the observation vislets pointing south are in accord with the movement, so that the resulting predicted trajectory is not decelerating as in the other cases, but accelerating toward south.



%(first column) and south (second column) do have a role in the trajectory prediction, being the related trajectories drifting themselves toward north and south. Interestingly, there is a general deceleration: this is the type of dynamics that happens when a person, while walking, turn his head to an object of interest, and changes direction slowing down to better look at it. Notably, all the vislets points have a distance which is somewhat constant (similar to $r$): this indicates that the LSTM has also captured the (artificial) distance between tracklet and vislet points. The unlikely vislet sequence (the red one, right column) lets the system predicts a fast trajectory with the vislets diverging from the trajectory. 

%Fig.~\ref{fig:Qualitative} second row
%30 1351  
%shows a %
%-->211359 - 563047
%similar behavior, going left to right: the purple sequence decelerate a little and goes north, the black one goes south.  

%Fig.~\ref{fig:Qualitative} third row 
%211239 
%shows that, for the individual going south, enforcing the head pose look north slows down dramatically the sequence, while looking south let the individual continue to go in that direction, while the correct trajectory was drifting left.




%%5935 4063 5215

\renewcommand{\arraystretch}{2}
\begin{table}[!b]
  \centering
  \caption{MAD errors on the different datasets including the requested (in bold) MX-LSTM-HPE \emph{Train and Test} and \emph{pace} MX-LSTM}
  \label{table:step}
  \resizebox{.999\linewidth}{!}{\begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Dataset}    & \textbf{MX-LSTM}  & \textbf{\begin{tabular}[c]{@{}c@{}}MX-LSTM-HPE\vspace{-7pt}\\ \textit{Train and Test}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\textit{pace}\vspace{-7pt}\\ \textit{MX-LSTM}\end{tabular}}\\ \hline
    \textbf{Zara01}     &  0.59   &  0.68       &    0.69      \\ \hline
    \textbf{Zara02}     &  0.35   &  0.51     &    0.73            \\ \hline
    \textbf{UCY}        &  0.49   &  0.58               &    0.59          \\ \hline
    \textbf{Town Centre} & 1.15   &  1.43               & 1.50                \\ \hline
  \end{tabular}}
\end{table}
\renewcommand{\arraystretch}{1}



\vspace{-0.2cm}


\vspace{-0.1cm}
    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/VFOA.png}
		\caption{VFOA pooling: For a given subject, he will try to avoid collision with the people who are inside is view frustum (blue circle). Others (red circle), will not influence his trajectory as they are no in his view frustum.}\label{fig:vfoaPoolingIllustration}
		\vspace{-15pt}
	\end{center}
    \end{figure*}











% \iffalse
% \begin{table*}[t]
%   \centering
%   \vspace{10em}
%   \caption{MAD -- Complete table: filled by Irtiza}
%   \label{xx-}
%   \scalebox{.88}{
%   \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
%     \hline
%     Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
%     \hline
%     Zara01    &2.74  &2.88  &0.90  &0.89  &0.58  &0.63  &0.68  &0.66  &0.69 &0.63 &0.60 &0.60 \\
%     \hline
%     Zara02    &2.23  &2.32  &1.1  &0.89  &1.2  &0.72  &0.63  &0.48  &0.43 &0.36 &0.41 &0.35  \\
%     \hline
%     UCY        &2.49  &2.57  &0.67  &0.54  &0.84  &0.53  &0.62  &0.60  &0.58 &0.51 &0.54 &0.49  \\
%     \hline
%     TownCentre &  &  &4.62  &1.96  &2.67  &2.09  &1.96  &1.7  &1.9 &1.7 &1.4 &1.15  \\
%     \hline \hline
%     TownCentre (real HPE) &--  & --  &--  &2.08  &--  &2.18  &--  &1.7  &-- &1.7 &1.44 &1.2  \\
%     \hline
%   \end{tabular}
%   }
%   \caption{FAD -- Complete table: filled by Irtiza}
%   \label{xx-}
%   \scalebox{.88}{
%   \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
%     \hline
%     Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
%     \hline
%     Zara01    &5.55  &5.55  &1.85  &1.81  &1.28  &1.37  &1.53  &1.51  &1.5 &1.40 &1.51 &1.31  \\
%     \hline
%     Zara02    &4.35  &4.35  &2.15  &1.90  &2.69  &1.56  &1.43  &1.06  &1.0 &0.84 &1.00 &0.79  \\
%     \hline
%     UCY        &4.66  &4.62  &1.39  &1.15  &1.92  &1.16  &1.40  &1.36  &1.27 &1.15 &1.23 &1.12  \\
%     \hline
%     TownCentre &  &  &8.26  &3.96  &5.15  &4.0  &3.96  &3.6  &4.2 &3.4 &2.9 &2.3  \\
%     \hline \hline
%     TownCentre (real HPE) &--  &--  &--  &4.12  &--  &4.2  &--  &3.6  &-- &3.4 &3.0 &2.36  \\
%     \hline
%   \end{tabular}
%   }
% \end{table*}







% \fs{TO DO:
% \begin{itemize}
%     \item show the qualitative sequences in the text and show the distributions of LSTM, vislet LSTM (original data) and the distribution of the vislets
%     \item 
% \end{itemize}}
% \fi


==> sections/experiments_v0.tex <==
\section{Experiments}\label{sec:experiments}
%% introduction
The experiments are quantitative and qualitative. The former evaluate MX-LSTM and some variants on 4 datasets (the 3 UCY sequences Zara01, Zara02 and UCY~\cite{lerner2007crowds}, and the Town Centre dataset~\cite{benfold2011stable}); all the sequences have ground truth head poses, while on the Town Centre we manually added ground truth head poses and head poses estimated by~\cite{}. In all the cases,  the head poses are expressed as pan angles over the 360 circle. Comparative approaches are: Social Force model (SF)~\cite{}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}; in addition we use a vanilla LSTM model as baseline, removing the social pooling from the S-LSTM.

Qualitative results unveil the interplay between tracklets and vislets that the MX-LSTM has learnt. 


\subsection{Qualitative results}
Fig.~\ref{fig:Qualitative} shows some qualitative results on the Zara~02 dataset. \emph{More results on the additional material}.
The first three rows of Fig.~\ref{fig:Qualitative}a) analyze the Individual-MX-LSTM, in which no social pooling is taken into account. Therefore, here each pedestrian is not influenced by the surrounding people, and the relationship between the tracklets and the vislets in the prediction can be observed without any confounding factor. 

    \begin{figure*}[h!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/Qualitative4.pdf}
		\caption{Qualitative results: a) Individual-MX-LSTM  b) MX-LSTM (better in color).}\label{fig:Qualitative}
	\end{center}
    \end{figure*}
    
These figures show different types of trajectories, each one equipped with its own vislets, here represented by the tip of the arrows: the blue one, which represents the routing input sequence given to the MX-LSTM. The green one is the ground-truth that has to be predicted. The yellow one is the prediction by MX-LSTM. The magenta one (left column) has been obtained by enforcing the vislets of the routing input sequence to point north (w.r.t. the image plane). The black one (center column) is the same as the magenta one, but pointing north. The red one (right column) has randomly placed vislets. The rationale of these last three types of sequences is to evaluate whether a different head pose behavior could trigger a diverse trajectory prediction. 

Fig.~\ref{fig:Qualitative} first row shows that actually vislets pointing north (first column) and south (second column) do have a role in the trajectory prediction, being the related trajectories drifting themselves toward north and south. Interestingly, there is a general deceleration: this is the type of dynamics that happens when a person, while walking, turn his head to an object of interest, and changes direction slowing down to better look at it. Notably, all the vislets points have a distance which is somewhat constant (similar to $r$): this indicates that the LSTM has also captured the (artificial) distance between tracklet and vislet points. The unlikely vislet sequence (the red one, right column) lets the system predicts a fast trajectory with the vislets diverging from the trajectory. 

Fig.~\ref{fig:Qualitative} second row
%30 1351  
c) shows a %
%-->211359 - 563047
similar behavior, going left to right: the purple sequence decelerate a little and goes north, the black one goes south.  

Fig.~\ref{fig:Qualitative} third row 
%211239 
shows that, for the individual going south, enforcing the head pose look north slows down dramatically the sequence, while looking south let the individual continue to go in that direction, while the correct trajectory was drifting left.


In Fig.~\ref{fig:Qualitative}b) the MX-LSTM is employed: a group scenario is taken into account, with the attention focused on the girl in the bottom-left corner. In the left column, the green ground truth arrows shows that the girl is conversing with the group members, with a movement close to 0 and the pan head angle which oscillates. In magenta, the behavior of the S-LSTM, predicting erroneously the girl leaving the group. This problem is important also looking at the analysis of Sec.\ref{sec:dataset}, which shows that when people are moving slowly or are static, forecasting error are in general dramatic.

In the central column, the MX-LSTM has been learnt the pattern of looking at the different speakers when in a group, with oscillating vislets, and almost no movement. 


In the case the vislets of the MX-LSTM are artificially enforced to go left (third column, cyan trajectories and arrows), the predicted trajectory is also developing in that direction, exhibiting a leave-group behavior.


%%5935 4063 5215







\subsection{Quantitative results}

%% Oracle experiments

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets.}
%   \label{tab:res-oracle}
%   \begin{tabular}{|c|l|*{6}{C{.092\textwidth}|}}
%     \hline
%     Metric & Dataset    &  SF  &  LTA   &  LSTM  & S-LSTM & MX-LSTM  & {\it MX-LSTM (real HPE)} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara 01 & 2.88 & 2.74 & 0.90 & 0.68 & {\bf 0.60} & {\it 0.80} \\
%     \cline{2-8}
%     & Zara 02    & 2.32 & 2.23 & 1.09 & 0.63 & {\bf 0.35} & {\it 0.37} \\
%     \cline{2-8}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & {\bf 0.49} & {\it 0.55} \\
%     \cline{2-8}
%     & TownCentre &9.35 &9.14   & 4.62 & 1.96 & {\bf 1.15} & {\it 1.21} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara 01 & 5.55 & 5.55 & 1.85 & 1.53 & {\bf 1.31} & {\it 1.61} \\
%     \cline{2-8}
%     & Zara 02    &  4.35 &  4.35 & 2.15 & 1.43 & {\bf 0.79} & {\it 0.82} \\
%     \cline{2-8}
%     & UCY        &  4.62 &  4.66 & 1.39 & 1.40 & {\bf 1.12} & {\it1.20 } \\
%     \cline{2-8}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & {\bf 2.30} & {\it 2.38} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

% \vspace{1em}
We evaluate our model against three different state-of-the-art methods: Social Force model (SF)~\cite{}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}; in addition we use an LSTM network that models each trajectory independently as baseline.
For all these methods, we used public released implementations, trying to replicate the results already published in previous papers. 
Discrepancies with the previous publications are mostly due to the evaluation protocol; in our case we use metric coordinates and the results are provided in meters.

Experiments follow the well established evaluation protocol proposed in~\cite{pellegrini2009iccv}.
A trajectory is ``observed'' for 8 frames and then the algorithm predicts the trajectory for the next 12 frames. Ground truth annotations are provided as inputs in the first 8 frames.
Two metrics are used to compare the prediction performances: Mean Average Displacement (MAD) error, which is the mean euclidean distance over all estimated points at each time-step in the predicted trajectories and the true trajectories, and Final Average Displacement (FAD) error, defined as the mean euclidean distance between the ﬁnal predicted locations and the ﬁnal true locations in the last predicted frame.
For the three UCY sequences three models have been trained: for each one we used two sequences as training data and then we tested on the third sequence. For Town Centre dataset the model has been trained and tested on the respective provided sets.

Quantitative results are reported in Table~\ref{tab:res-oracle}.
The MX-LSTM outperforms the state-of-the-art methods in every single sequence and with both the metrics: The highest gain is achieved in Town Centre dataset, an extremely crowded scenario where complex non-linear paths are mostly caused by human-human interactions. Our MX-LSTM and S-LSTM are both able to capture these kind of interactions, but our approach models better the situation by leveraging the head pose.
Please note that different methods rely on different input data: in addition to the location of each pedestrian in the scene at each time-step, SF and LTA require the destination point of each individual, ... require annotation about social groups, and our MX-LSTM require the head pose of each individual for every frame in the observation period. 
%We will discuss below how our method performs with a real head pose estimator instead of oracle information.
% Our method relies on the information about the head pose for the observation period. 
To perform fair comparison with the state-of-the-art methods, we did experiments feeding the method with the head poses estimated by ...~\cite{}.
We report here experiments only on the Town Centre dataset, wich is the only one that provides bounding box annotations for pedestrians and heads. The last row of the table shows how our proposed MX-LSTM is extremely robust to head pose errors, with an average drop in performances of about 5(?)\%.



%% Ablation study
% \subsubsection*{Ablation study}

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on all the datasets for three variations of the proposed MX-LSTM method. The last column reports the results of the proposed model to ease the comparison.}
%   \label{tab:res-variations}
%   \begin{tabular}{|c|l|*{4}{C{.095\textwidth}|}}
%     \hline
%     Metric & Dataset    &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara 01 & 0.63 & 0.63 & 0.60 & {\bf 0.60} \\
%     \cline{2-6}
%     & Zara 02    & 0.72 & 0.36 & 0.41 & {\bf 0.35} \\
%     \cline{2-6}
%     & UCY        & 0.53 & 0.51 & 0.54 & {\bf 0.49} \\
%     \cline{2-6}
%     & TownCentre & 2.09 & 1.70 & 1.40 & {\bf 1.15} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 2.18} & {\it 1.70} & {\it 1.44} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara 01 & 1.37 & 1.40 & 1.51 & {\bf 1.31} \\
%     \cline{2-6}
%     & Zara 02    & 1.56 & 0.84 & 1.00 & {\bf 0.79} \\
%     \cline{2-6}
%     & UCY        & 1.16 & 1.15 & 1.23 & {\bf 1.12} \\
%     \cline{2-6}
%     & TownCentre & 4.00 & 3.40 & 2.90 & {\bf 2.3} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 4.20} & {\it 3.40} & {\it 3.0} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

%\fs{I would move here Section 4. If this is ok for you, I will move and adapt the text here soon}
We investigate three variations of the MX-LSTM to capture the net contributions of the different aspects that characterize it. They are:\\
\textbf{Unmixed LSTM}: it serves to highlight the importance of enforcing the LSTM to jointly studying the separated information streams, tracklets and vislets, through the full covariance. Essentially, instead of learning the $4\times4$ full $\mathbf{\Sigma}$, the approach estimates two bidimensional covariances\footnote{The 2x2 covariance is estimated employing two variances $\sigma_1, \sigma_2$ and a correlation terms $\rho$ as presented in \cite{graves2013generating} Eq.(24) and (25).} $\mathbf{\Sigma}_x$ and $\mathbf{\Sigma}_a$ for the trajectory and the vislet modeling respectively, without capturing the cross-stream covariances. The equations that change w.r.t. MX-LSTM are Eq. (\ref{eq:LLog}) and (\ref{eq:params}), which become, respectively, 
\begin{eqnarray}
L^i(\mathbf{W}_{x},\mathbf{W}_{a},\mathbf{W}_H,\mathbf{W}_{\text{LSTM}},\mathbf{W}_{o}) &=&\nonumber\\  -\sum_{T_{obs}+1}^{T_{pred}}log\left( P([\mathbf{x}^{(i)}_t]^T|\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t \right)+\!\!\\\nonumber
log\left(P([\mathbf{a}^{(i)}_t]^T|\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t\right)
\end{eqnarray}
where $\bo{\mu}^{(x,i)}_t=[{}_x\mu^{(x,i)}_t,{}_y\mu^{(x,i)}_t]$ and the same apply for the variance vector;
\begin{equation}
[\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t,\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t]^T \!=\! \mathbf{W}_o \mathbf{h}^{(i)}_{t-1}\label{eq:params}
\end{equation}\\
\textbf{noFrustum MX-LSTM}: this variation of the MX-LSTM uses the social pooling as in~\cite{alahi2016cvpr}, in which the interest area where persons' hidden states $\{\mathbf{h}^{j}_t\}$ are pooled into the social tensor is all around the individual. In other words, no frustum selecting the people that have to be considered is used here.\\
\textbf{Individual MX-LSTM}: In this case, no social pooling is taken into account, therefore the embedding operation of Eq.~(\ref{eq:pooling}) is absent, and the weight matrix $\mathbf{W}_H$ vanishes. In practice, this variant learns independent models for each person, each one of them is considering the tracklet and vislet points.

Table~\ref{tab:res-variations} reports numerical results for all the variations on all the datasets. 
Again, although the complete method always outperforms all the competitors, the highest improvement is on the Town Centre sequence. In our opinion this is due to the different level of complexity in the data, indeed most of the trajectories in UCY sequences are relatively linear, with poor social interactions, while in Town Centre there are many interactions like forming and splitting groups, and crossing trajectories.
For the same reason, this is also the only dataset where the introduction of the view frustum in the pooling of social interactions gives the highest benefits. In all the sequences instead, decoupling the covariance matrix into a block diagonal matrix leads to a sensitive increase in the prediction error; this proves the tight relation between the head orientation and the motion of an individual.



% \subsection*{Validation with a real HPE}

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on the Town Centre dataset for the four variants of the proposed approach feeded with oracle information and real head pose estimations.}
%   \label{tab:res-real}
%   \begin{tabular}{|c|l|*{4}{C{.1\textwidth}|}}
%     \hline
%     Metric & Inputs &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{2}{.14\textwidth}{\centering Mean Average Displacement} & Oracle & 2.09 & 1.70 & 1.40 &  \\
%     \cline{2-6}
%     & HPE~\cite{hpe} & 2.18 & 1.70 & 1.44 &  \\
%     \hline \hline
%     \multirow{2}{.14\textwidth}{\centering Final Average Displacement} & Oracle & 4.00 & 3.40 & 2.90 &  \\
%     \cline{2-6}
%     & HPE~\cite{hpe} & 4.20 & 3.40 & 3.00 &  \\
%     \hline
%   \end{tabular}
% \end{table*}

% Our method relies on the information about the head pose for the observation period. To provide a fair comparison with the state-of-the-art methods, we did experiments feeding the method with the output of the ... head pose estimation~\cite{}.
% We provide here experiments only on the Town Centre dataset wich is the only one that provides bounding box annotations for pedestrians and heads.
% Table~\ref{tab:res-real} shows how our proposed MX-LSTM is extremely robust to head pose errors, with an average drop in performances of about 5(?)\%.


\iffalse
\begin{table*}[t]
  \centering
  \vspace{10em}
  \caption{MAD -- Complete table: filled by Irtiza}
  \label{xx-}
  \scalebox{.88}{
  \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
    \hline
    Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
    \hline
    Zara 01    &2.74  &2.88  &0.90  &0.89  &0.58  &0.63  &0.68  &0.66  &0.69 &0.63 &0.60 &0.60 \\
    \hline
    Zara 02    &2.23  &2.32  &1.1  &0.89  &1.2  &0.72  &0.63  &0.48  &0.43 &0.36 &0.41 &0.35  \\
    \hline
    UCY        &2.49  &2.57  &0.67  &0.54  &0.84  &0.53  &0.62  &0.60  &0.58 &0.51 &0.54 &0.49  \\
    \hline
    TownCenter &  &  &4.62  &1.96  &2.67  &2.09  &1.96  &1.7  &1.9 &1.7 &1.4 &1.15  \\
    \hline \hline
    TownCenter (real HPE) &--  & --  &--  &2.08  &--  &2.18  &--  &1.7  &-- &1.7 &1.44 &1.2  \\
    \hline
  \end{tabular}
  }
  \caption{FAD -- Complete table: filled by Irtiza}
  \label{xx-}
  \scalebox{.88}{
  \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
    \hline
    Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
    \hline
    Zara 01    &5.55  &5.55  &1.85  &1.81  &1.28  &1.37  &1.53  &1.51  &1.5 &1.40 &1.51 &1.31  \\
    \hline
    Zara 02    &4.35  &4.35  &2.15  &1.90  &2.69  &1.56  &1.43  &1.06  &1.0 &0.84 &1.00 &0.79  \\
    \hline
    UCY        &4.66  &4.62  &1.39  &1.15  &1.92  &1.16  &1.40  &1.36  &1.27 &1.15 &1.23 &1.12  \\
    \hline
    TownCenter &  &  &8.26  &3.96  &5.15  &4.0  &3.96  &3.6  &4.2 &3.4 &2.9 &2.3  \\
    \hline \hline
    TownCenter (real HPE) &--  &--  &--  &4.12  &--  &4.2  &--  &3.6  &-- &3.4 &3.0 &2.36  \\
    \hline
  \end{tabular}
  }
\end{table*}







\fs{TO DO:
\begin{itemize}
    \item show the qualitative sequences in the text and show the distributions of LSTM, vislet LSTM (original data) and the distribution of the vislets
    \item 
\end{itemize}}
\fi

==> sections/experiments_v1.tex <==
\vspace{-0.1cm} \section{Experiments}\label{sec:experiments}


\todo{

\begin{itemize}
\item New experiments to be added
\item Analysis of new experiments to bew drawn
\end{itemize}
}
%% introduction
% The experiments are quantitative and qualitative. The former evaluate MX-LSTM and some variants on 4 datasets (the 3 UCY sequences Zara01, Zara02 and UCY~\cite{lerner2007crowds}, and the Town Centre dataset~\cite{benfold2011stable}); all the sequences have ground truth head poses, while on the Town Centre we manually added ground truth head poses and head poses estimated by~\cite{}. In all the cases,  the head poses are expressed as pan angles over the 360 circle. Comparative approaches are: Social Force model (SF)~\cite{}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}; in addition we use a vanilla LSTM model as baseline, removing the social pooling from the S-LSTM.
\vspace{-0.1cm}
We present here both quantitative and qualitative experiments.
Quantitative results validate the proposed MX-LSTM model, setting the new state-of-the-art for trajectory forecasting; results are also provided for an ablation study showing the importance of the different parts of the MX-LSTM. Finally, we present the very first results on head pose forecasting. Qualitative results unveil the interplay between tracklets and vislets that the MX-LSTM has learnt. 


% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets. The first 5 columns are the comparative methods and our proposed model trained and tested with GT annotations. MX-LSTM-HPE  is our model %trained with ground truth annotations and
%   tested with the output of a real head pose estimator~\cite{lee2015fast}. The last 3 columns are variations of our approach trained and tested on GT annotations.}
%   \label{tab:res-oracle}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{|c|l *{5}{|C{.093\textwidth}} !{\vrule width 2pt} C{.093\textwidth} !{\vrule width 2pt} *{3}{C{.093\textwidth}|}}
%     %\hhline{--------||---}
%     \hline
%     Metric & Dataset    &  SF~\cite{yamaguchi2011cvpr}  &  LTA~\cite{pellegrini2009iccv}   &  Vanilla LSTM~\cite{alahi2016cvpr}  & Social LSTM~\cite{alahi2016cvpr} & MX-LSTM  & {\it MX-LSTM-HPE } & Individual MX-LSTM  &  NoFrustum MX-LSTM  &  BD- MX-LSTM   \\
%     % \hhline{========::===}
%     \hline \hline
%     \multirow{5}{*}{\centering MAD} & Zara01 & 2.88 & 2.74 & 0.90 & 0.68 & {\bf 0.59} & {\bf\emph{0.66}} & 0.63 & 0.63 & 0.60 \\
%     %\hhline{ -------||---}
%     \cline{2-11}
%     & Zara02     & 2.32 & 2.23 & 1.09 & 0.63 & {\bf 0.35} & {\bf\emph{0.37}} & 0.72 & 0.36 & 0.41 \\
%     \cline{2-11}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & {\bf 0.49} & {\bf\emph{0.55}} & 0.53 & 0.51 & 0.54 \\
%     \cline{2-11}
%     & TownCentre &9.35 &9.14   & 4.62 & 1.96 & {\bf 1.15} & {\bf\emph{1.21}} & 2.09 & 1.70 & 1.40 \\
%     % \hhline{========::===}
%     \hline \hline
%     \multirow{5}{*}{\centering FAD} & Zara01 & 5.55 & 5.55 & 1.85 & 1.53 & {\bf 1.31} & {\bf\emph{1.43}} & 1.37 & 1.40 & 1.51 \\
%     \cline{2-11}
%     & Zara02     & 4.35 &  4.35 & 2.15 & 1.43 & {\bf 0.79} & {\bf\emph{0.82}} & 1.56 & 0.84 & 1.00 \\
%     \cline{2-11}
%     & UCY        & 4.62 &  4.66 & 1.39 & 1.40 & {\bf 1.12} & {\bf\emph{1.20}} & 1.16 & 1.15 & 1.23 \\
%     \cline{2-11}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & {\bf 2.30} & {\bf\emph{2.38}} & 4.00 & 3.40 & 2.90 \\
%     %\hhline{--------||---}
%     \hline
%   \end{tabular}
%   }
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets. The first 5 columns are state-of-the-art methods and our proposed model trained and tested with ground truth annotations. Column 6 is our model trained with ground truth annotations and tested with the output of a real head pose estimator~\cite{lee2015fast}. Columns 7-9 are variations of our approach trained and tested on annotated data.}
%   \label{tab:res-oracle}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{|c|l *{9}{|C{.093\textwidth}} |}% !{\vrule width 2pt} *{3}{C{.093\textwidth}|}}
%     %\hhline{--------||---}
%     \hline
%     Metric & Dataset    &  SF~\cite{yamaguchi2011cvpr}  &  LTA~\cite{pellegrini2009iccv}   &  Vanilla LSTM~\cite{alahi2016cvpr}  & Social LSTM~\cite{alahi2016cvpr}  & Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM & MX-LSTM & {\it MX-LSTM (real HPE)} \\
%     \hline \hline
%     \multirow{4}{*}{\centering MAD}
%     & Zara01     & 2.88 & 2.74 & 0.90 & 0.68 & 0.63 & 0.63 & 0.60 & {\bf 0.59} & {\it 0.66} \\
%     \cline{2-11}
%     & Zara02     & 2.32 & 2.23 & 1.09 & 0.63 & 0.72 & 0.36 & 0.41 & {\bf 0.35} & {\it 0.37} \\
%     \cline{2-11}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & 0.53 & 0.51 & 0.54 & {\bf 0.49} & {\it 0.55} \\
%     \cline{2-11}
%     & TownCentre & 9.35 & 9.14 & 4.62 & 1.96 & 2.09 & 1.70 & 1.40 & {\bf 1.15} & {\it 1.21} \\
%     \hline \hline
%     \multirow{4}{*}{\centering FAD} 
%     & Zara01     &  5.55 &  5.55 & 1.85 & 1.53 & 1.37 & 1.40 & 1.51 & {\bf 1.31} & {\it 1.43} \\
%     \cline{2-11}
%     & Zara02     &  4.35 &  4.35 & 2.15 & 1.43 & 1.56 & 0.84 & 1.00 & {\bf 0.79} & {\it 0.82} \\
%     \cline{2-11}
%     & UCY        &  4.62 &  4.66 & 1.39 & 1.40 & 1.16 & 1.15 & 1.23 & {\bf 1.12} & {\it 1.20} \\
%     \cline{2-11}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & 4.00 & 3.40 & 2.90 & {\bf 2.30} & {\it 2.38} \\
%     \hline
%   \end{tabular}
%   }
% \end{table*}







% \subsection{Quantitative results}

%% Oracle experiments

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets.}
%   \label{tab:res-oracle}
%   \begin{tabular}{|c|l|*{6}{C{.093\textwidth}|}}
%     \hline
%     Metric & Dataset    &  SF~\cite{yamaguchi2011cvpr}  &  LTA~\cite{pellegrini2009iccv}   &  Vanilla LSTM~\cite{alahi2016cvpr}  & Social LSTM~\cite{alahi2016cvpr} & MX-LSTM  & {\it MX-LSTM (real HPE)} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara01 & 2.88 & 2.74 & 0.90 & 0.68 & {\bf 0.59} & {\it 0.66} \\
%     \cline{2-8}
%     & Zara02    & 2.32 & 2.23 & 1.09 & 0.63 & {\bf 0.35} & {\it 0.37} \\
%     \cline{2-8}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & {\bf 0.49} & {\it 0.55} \\
%     \cline{2-8}
%     & TownCentre &9.35 &9.14   & 4.62 & 1.96 & {\bf 1.15} & {\it 1.21} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara01 & 5.55 & 5.55 & 1.85 & 1.53 & {\bf 1.31} & {\it 1.43} \\
%     \cline{2-8}
%     & Zara02    &  4.35 &  4.35 & 2.15 & 1.43 & {\bf 0.79} & {\it 0.82} \\
%     \cline{2-8}
%     & UCY        &  4.62 &  4.66 & 1.39 & 1.40 & {\bf 1.12} & {\it1.20 } \\
%     \cline{2-8}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & {\bf 2.30} & {\it 2.38} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

\subsection{Quantitative results}\label{sec:quantitative}\vspace{-0.1cm}
We evaluate our model against all the published approaches which made their code publicly available: %\footnote{We will do the same upon acceptance.}: 
%three different state-of-the-art methods: 
Social Force model (SF)~\cite{yamaguchi2011cvpr}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, Vanilla LSTM and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}.

%in addition we use a Vanilla LSTM  network that models each trajectory independently as baseline.
%For all these methods, we used public released implementations.
%, trying to replicate the results already published in previous papers. 
%Discrepancies with the previous publications are mostly due to the evaluation protocol; in our case we use metric coordinates and the results are provided in meters.
Experiments follow the widely-used evaluation protocol of~\cite{pellegrini2009iccv}, in which the algorithm first observes 8 ``observation'' ground truth (GT) frames of a trajectory, predicting the following 12 ones. 
%the well established evaluation protocol proposed in~\cite{pellegrini2009iccv}.
%A trajectory is ``observed'' for 8 frames and then the algorithm predicts the trajectory for the next 12 frames. Ground truth annotations are provided as inputs in the first 8 frames.
For the three UCY sequences three models have been trained: for each one we used two sequences as training data and then we tested on the third sequence. For Town Centre dataset the model has been trained and tested on the respective provided sets. The grid for the social pooling (Eq.~\eqref{eq:social}) has $N_o\times N_o$ cells with $N_o=32$.
The view frustum aperture angle has been cross-validated on the training partition of the TownCenter and kept fixed for the remaining trials ($\gamma=40^{\circ}$), while the depth $d$ is simply bounded by the social pooling grid. 
Trajectory prediction performances are analyzed with the Mean Average Displacement (MAD) error (euclidean distance between predicted and GT points, averaged over the sequence), and Final Average Displacement (FAD) error (distance between the last predicted point and the corresponding GT point)~\cite{pellegrini2009iccv}.
%Two metrics are used to compare the prediction performances: Mean Average Displacement (MAD) error, which is the mean euclidean distance over all estimated points at each time-step in the predicted trajectories and the true trajectories, and Final Average Displacement (FAD) error, defined as the mean euclidean distance between the ﬁnal predicted locations and the ﬁnal true locations in the last predicted frame.


Results are reported in Table~\ref{tab:res-oracle}.
The MX-LSTM outperforms the state-of-the-art methods in every single sequence and with both  metrics, with an average improvement of 32.7\%. The highest relative gain is achieved in Zara02 dataset, where complex non-linear paths are mostly caused by standing conversational groups and people that walk close to them, avoiding collisions. People slowing down and looking at the window shops pose also a challenge. As shown in Fig.~\ref{fig:angles}, slow moving and interacting pedestrians cause troubles to the competing methods, while MX-LSTM clearly overcomes such shortcomings denoting a better model. Qualitative motivations will follow in Sec.~\ref{sec:qualitative}.


%Our MX-LSTM and S-LSTM are both able to capture these kind of interactions, but our approach models better the situation by leveraging the head pose.
Please note that different methods rely on different input data: 
%in addition to the location of each pedestrian in the scene at each time-step, 
both SF and LTA require the destination point of each individual, while SF also requires annotations about social groups; MX-LSTM requires the head pose of each individual for the first 8 frames, but this can be estimated by a head pose estimator. This motivates our next experiment: we automatically estimate the head bounding box given the feet positions on the floor plane, assuming  people being $1.80$m tall. Then, we apply the head pose estimator of~\cite{lee2015fast} which gives continuous angles that can be used as input of our approach now named ``MX-LSTM-HPE''.   
%We will discuss below how our method performs with a real head pose estimator instead of oracle information.
% Our method relies on the information about the head pose for the observation period. 
%To perform fair comparison with the state-of-the-art methods, we also performed experiments feeding the model with the head poses estimated by \cite{lee2015fast} at testing time.
%We report here experiments only on the Town Centre dataset, wich is the only one that provides bounding box annotations for pedestrians and heads. 
As shown by the scores in Table~\ref{tab:res-oracle}, MX-LSTM-HPE does not suffer about small errors in the input head pose, with an average drop in performances of only 5\%. Note that MX-LSTM-HPE still outperforms all competing methods on all dataset even with the noisy estimated head pose information.

How accurate should the head pose estimation be, for the MX-LSTM-HPE to have convincing performances, for example outperforming the Social LSTM? We answer this question by corrupting the true head pose estimate with additive Gaussian noise$\sim\mathcal{N}(\alpha_t,\hat{\sigma})$, where $\alpha_t$ is the correct head pose and $\hat{\sigma}$ the standard deviation. MX-LSTM-HPE outperforms social-LSTM up to a noise of $\hat{\sigma}=24^{\circ}$.

%We investigate how robust is the MX-LSTM in this sense, generating random head poses from a circular Gaussian distribution . We found that, on the UCY sequence, we can reach the S-LSTM performances (MAD $= 0.62$) with  (so we are correctly guessing just two directions), while with completely random head poses input we have an MAD error of $1.02$, still better than LTA and SF. 



%% Ablation study
%\subsubsection*{Ablation study}

%% ----------------------------------
%%  two columns
%% ----------------------------------
% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on all the datasets for three variations of the proposed MX-LSTM method. The last column reports the results of the proposed model to ease the comparison.}
%   \label{tab:res-variations}
%   \begin{tabular}{|c|l|*{4}{C{.095\textwidth}|}}
%     \hline
%     Metric & Dataset    &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara01 & 0.63 & 0.63 & 0.60 & {\bf 0.59} \\
%     \cline{2-6}
%     & Zara02    & 0.72 & 0.36 & 0.41 & {\bf 0.35} \\
%     \cline{2-6}
%     & UCY        & 0.53 & 0.51 & 0.54 & {\bf 0.49} \\
%     \cline{2-6}
%     & TownCentre & 2.09 & 1.70 & 1.40 & {\bf 1.15} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 2.18} & {\it 1.70} & {\it 1.44} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara01 & 1.37 & 1.40 & 1.51 & {\bf 1.31} \\
%     \cline{2-6}
%     & Zara02    & 1.56 & 0.84 & 1.00 & {\bf 0.79} \\
%     \cline{2-6}
%     & UCY        & 1.16 & 1.15 & 1.23 & {\bf 1.12} \\
%     \cline{2-6}
%     & TownCentre & 4.00 & 3.40 & 2.90 & {\bf 2.3} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 4.20} & {\it 3.40} & {\it 3.0} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

%% ----------------------------------
%%  single column
%% ----------------------------------
% \begin{table}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) on all the datasets for three variations of the proposed MX-LSTM method. The last column reports the results of the proposed model to ease the comparison.}
%   \label{tab:res-variations}
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{|c|l|*{4}{C{.093\textwidth}|}}
%     \hline
%     Metric & Dataset    &  Individual MX-LSTM  &  noFrustum MX-LSTM  &  Unmixed LSTM  &  MX-LSTM \\
%     \hline \hline
%     \multirow{4}{*}{\centering MAD} & Zara01 & 0.63 & 0.63 & 0.60 & {\bf 0.59} \\
%     \cline{2-6}
%     & Zara02    & 0.72 & 0.36 & 0.41 & {\bf 0.35} \\
%     \cline{2-6}
%     & UCY        & 0.53 & 0.51 & 0.54 & {\bf 0.49} \\
%     \cline{2-6}
%     & TownCentre & 2.09 & 1.70 & 1.40 & {\bf 1.15} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 2.18} & {\it 1.70} & {\it 1.44} & {\it 1.21} \\
%     \hline \hline
%     \multirow{4}{*}{\centering FAD} & Zara01 & 1.37 & 1.40 & 1.51 & {\bf 1.31} \\
%     \cline{2-6}
%     & Zara02    & 1.56 & 0.84 & 1.00 & {\bf 0.79} \\
%     \cline{2-6}
%     & UCY        & 1.16 & 1.15 & 1.23 & {\bf 1.12} \\
%     \cline{2-6}
%     & TownCentre & 4.00 & 3.40 & 2.90 & {\bf 2.3} \\
%     % \cline{2-6}
%     % & {\it TownCenter (real HPE)} & {\it 4.20} & {\it 3.40} & {\it 3.0} & {\it 2.38} \\
%     \hline
%   \end{tabular}
%   }
% \end{table}
\vspace{-0.2cm}
\subsubsection{Ablation study}\label{sec:ablation}
Aside with the models in the literature, we investigate three variations of the MX-LSTM to capture the net contributions of the different parts that characterize our approach.

\noindent\textbf{Block-Diagonal MX-LSTM (BD-MX-LSTM)}: it serves to highlight the importance of estimating full covariances to understand the interplay between tracklets and vislets.  
%
%enforcing the LSTM to jointly studying the separated information streams, tracklets and vislets, through the full covariance. Essentially, instead of learning the $4\times4$ full $\mathbf{\Sigma}$, 
%
Essentially, the approach estimates two bidimensional covariances\footnote{The $2\times2$ covariance is estimated employing two variances $\sigma_1, \sigma_2$ and a correlation terms $\rho$ as presented in \cite{graves2013generating} Eq.(24) and (25).} $\mathbf{\Sigma}_x$ and $\mathbf{\Sigma}_a$ for the trajectory and the vislet modeling respectively, without capturing the cross-stream covariances.

% \emph{The equations that differ w.r.t. MX-LSTM will be given as supplemental material.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
are Eq. (\ref{eq:LLog}) and (\ref{eq:params}), which become, respectively, 
\begin{eqnarray}
L^i(\mathbf{W}_{x},\mathbf{W}_{a},\mathbf{W}_H,\mathbf{W}_{\text{LSTM}},\mathbf{W}_{o}) &=&\nonumber\\  -\sum_{T_{obs}+1}^{T_{pred}}log\left( P([\mathbf{x}^{(i)}_t]^T|\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t \right)+\!\!\\\nonumber
log\left(P([\mathbf{a}^{(i)}_t]^T|\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t\right)
\end{eqnarray}
where $\bo{\mu}^{(x,i)}_t=[{}_x\mu^{(x,i)}_t,{}_y\mu^{(x,i)}_t]$ and the same apply for the variance vector;
\begin{equation}
[\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t,\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t]^T \!=\! \mathbf{W}_o \mathbf{h}^{(i)}_{t-1}\label{eq:params}
\end{equation}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{NoFrustum MX-LSTM}: this variation of the MX-LSTM uses social pooling as in~\cite{alahi2016cvpr}, in which the interest area where people hidden states $\{\mathbf{h}^{j}_t\}$ are pooled into the social tensor  all around the individual. In other words, no frustum selecting the people that have to be considered is used here.

\noindent\textbf{Individual MX-LSTM}: In this case, no social pooling is taken into account, therefore the embedding operation of Eq.~(\ref{eq:pooling}) is absent, and the weight matrix $\mathbf{W}_H$ vanishes. In practice, this variant learns independent models for each person, each one considering the tracklet and vislet points.

\vspace{1em}
Table~\ref{tab:res-oracle}, last three columns, reports numerical results for all the MX-LSTM simplifications on all the datasets. The main facts that emerge are: 1) the highest variations are with the Zara02 sequence, where MX-LSTM doubles the performances of the worst approach (Individual MX-LSTM); 2) the worst performing is in general Individual MX-LSTM, showing that social reasoning is indeed necessary; 3) social reasoning is systematically improved with the help of the vislet-based view-frustum; 4) full covariance estimation has a role in pushing down the error which is already small with the adoption of vislets.  

Summarizing the results so far, having vislets as input allows to definitely increase the trajectory forecasting performance, even if vislets are estimated with noise. Vislets should be used to understand social interactions with social pooling, by building a view frustum that tells which are the people currently observed by each individual. All of these features are done efficiently by the MX-LSTM: in fact the training time is the same with having an LSTM with social pooling.


%Again, although the complete method always outperforms all the competitors, the highest improvement is on the TownCentre sequence. In our opinion this is due to the different level of complexity in the data, indeed most of the trajectories in UCY sequences are relatively linear, with poor social interactions, while in TownCentre there are many interactions like forming and splitting groups, and crossing trajectories.
%For the same reason, this is also the only dataset where the introduction of the view frustum in the pooling of social interactions gives the highest benefits. In all the sequences instead, %decoupling the covariance matrix into a block diagonal matrix 
%neglecting the interplay of position and gaze (Unmixed LSTM) leads to a sensitive increase in the prediction error; this proves the tight relation between the head orientation and the motion of an individual.


%\subsection*{Head pose prediction}
%\vspace{1em}
% Since MX-LSTM predicts the head pose too, we should have a quality measure on it. We propose two types of errors: the \emph{pose plausibility error} $e_{\text{pp}}$, which measures how much the head pose is compatible with the predicted trajectory, considering that we are not contortionists, and the \emph{angular error} $e_{\alpha}$, which evaluates the error of the predicted head pose angle with respect to the ground truth one.

% The $e_{\text{pp}}$ is computed in the following way (see Fig.~\ref{fig:explanations} for the notation): let $\Delta_\omega(t) = |\omega_{t,real}-\omega_{t,pred}|$, where $\omega_t$ is the angle between the vislet and the tracklets at time $t$. Then $e_{\text{pp}}=\min \left( \Delta_\omega(t),180 -\Delta_\omega(t)\right)$. Having a low $e_{\text{pp}}$ means to predict head poses that are anatomically plausible with the predicted movement.
\vspace{-0.2cm}
\subsubsection{Head pose forecasting}\vspace{-0.1cm}
As done with trajectories, we are also providing a forecast of the head pose of each individual at each frame which is a distinctive attribute of our method.   We evaluate the performances of this estimation in terms of mean angular error $e_{\alpha}$, which is the mean absolute difference between the estimated pose (angle $\alpha_{t,\cdot}$ in Fig.~\ref{fig:explanations}c) and the annotated GT.
%is equal to the pose plausibility error, with $\alpha_{t,\cdot}$ instead of $\omega_{t,\cdot}$. It tells how much the direction in which is looking an individual at a particular instant is different wrt the real direction, independently on where the individual has been predicted to be located. Having a low $e_{\alpha}$ means that in general we are guessing correctly the direction of interest, especially in coincidence with a low MAD, as it is in general in our experiments.   

% \begin{table}[t!]
%   \centering
%   \caption{Pose plausibility error ($e_{\text{pp}}$) and angular error ($e_{\alpha}$) for the MX-LSTM model on all the datasets.}
%   \label{tab:res-angle}
%   \begin{tabular}{|l|*{2}{C{.1\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     TownCentre &  23.30  &  26.48  \\
%     \hline
%   \end{tabular}
% \end{table}

\begin{table}[t!]
  \centering
  \small
  \caption{Mean angular error (in degrees) for the state-of-the-art head pose estimator~\cite{lee2015fast}, and the MX-LSTM model fed with GT annotations and estimated values (MX-LSTM-HPE).}
  \label{tab:res-angle}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{|l|*{4}{C{.06\textwidth}|}}
    \hline
    Metric                &  Zara01  &  Zara02  &   UCY   &  Town Centre \\
    \hline
    HPE~\cite{lee2015fast} & 14.29   &   20.02  &  19.90 &   25.08    \\   
    \hline
    MX-LSTM               &  12.98   &   20.55  &  21.36  &   26.48    \\
    \hline
    MX-LSTM-HPE  &  17.69   &   21.92  &  24.37  &   28.55  \\
    \hline
  \end{tabular}
  }
\end{table}





% \begin{table}[t!]
%   \centering
%   \begin{minipage}[t]{.39\columnwidth}
%     \centering
%     \caption{Head pose estimation errors for MX-LSTM on all the datasets (in degrees).}
%     \label{tab:res-angle}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{|l|*{2}{C{.25\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     Town Centre &  23.30  &  26.48  \\
%     \hline
%     \end{tabular}
%     }
%   \end{minipage}
%   \hspace{.02\linewidth}
%   \begin{minipage}[t]{.57\columnwidth}
%     \centering
%     \caption{Boh}
%     \label{fig:angle}
%     \includegraphics[width=\linewidth]{figure/supercool.pdf}
%   \end{minipage}
% \end{table}



Table~\ref{tab:res-angle} shows numerical results of the static head pose estimator~\cite{lee2015fast} (HPE), the MX-LSTM using GT head poses, and the MX-LSTM fed with the output of HPE during the observation period (MX-LSTM-HPE).
In all the cases our forecast output is comparable with the one of HPE, but in our case we do not use appearance cues -- i.e. we do not look at the images at all.
In case of Zara01, the MX-LSTM is even better that the static prediction showing the forecasting power of our model. In our opinion this is due to the fact that in this sequence trajectories are mostly very linear and fast, and heads are mostly aligned with the direction of motion. When we provide estimations to the MX-LSTM model during the observation period, angular error increases, as expected. Despite this, the error is surprisingly limited.
%The low error achieved in Zara01 is probably related to the fact that this sequence is dominated people moving linearly and fast, thus the head orientation is usually aligned with the trajectory and the model can learn this behavior very easily.
%Zara02: more complicate, people are standing more in between of people moving fast (right Irtiza?) so big variety of disalignments, and you have the biggest errors
%Zara02 is a more challenging sequence, since there is a high number of standing group formations in the middle of the scene; these trajectories are very noisy, and as a consequence $e_{\text{pp}}$ increase.
%UCY: still group formations, but they are moving, so less disalignment and noise, numbers are in accord with this (Irtiza agree?)
%In UCY, the grouping formations are still present, but in this case they are moving, so noise is reduced and thus the disalignement between trajectory and head pose.
\subsubsection{Horizon Effect}\label{sec:horizon}
\todo{ Explain the bullet points and place all the relevant tables
\begin{itemize}
    \item We show that MX-LSTM is also more accurate in long term forecasting;
    %the head pose, also given by a normal head pose estimator;\vspace{-5pt}
    \item we illustrate that social LSTM degrades as we increase the prediction interval
    \item We motivate that even with fewer observation interval the injection of head pose provides useful information in long term forecasting. 
    \item We present ranking order remains same in all experiment.
\end{itemize}
}
\subsection{Qualitative results}\label{sec:qualitative}
\vspace{-0.1cm}
    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/Qualitative8_theo.png}
		\caption{Qualitative results: a) MX-LSTM  b) Ablation qualitative study on Individual MX-LSTM (better in color).}\label{fig:Qualitative}
		\vspace{-15pt}
	\end{center}
    \end{figure*}

Fig.~\ref{fig:Qualitative} shows  qualitative results on the Zara02 dataset, which has been shown to be the most complex scenario in the quantitative experiments
%\footnote{Please check supplemental material for further results.}. 
%
Fig.~\ref{fig:Qualitative}a presents MX-LSTM results: a group scenario is taken into account, with the attention focused on the girl in the bottom-left corner. In the left column, the green ground-truth prediction vislets show that the girl is conversing with the group members, with a movement close to zero and the pan head angle which oscillates. In magenta, the behavior of the S-LSTM, predicting erroneously the girl leaving the group. This error confirms the problem of competing methods in forecasting the motion of people slowly moving or static as discussed in Sec.\ref{sec:dataset}, and further confirmed by the results of the quantitative experiments. %, which show that when people are moving slowly or are static, forecasting error are in general dramatic.
In the central column, the observation sequence given to the MX-LSTM is shown in orange (almost static with oscillating vislets). The related prediction (in yellow) shows oscillating vislets, and almost no movement, confirming that the MX-LSTM has learnt this particular social behavior. If we provide to MX-LSTM an artificial observation sequence with the annotated positions (real trajectory) but vislets oriented toward west  (third column, orange arrows), where no people are present, the MX-LSTM predicts a trajectory departing from the group (cyan trajectory and arrows).


The two rows of Fig.~\ref{fig:Qualitative}b) analyze the Individual MX-LSTM, in which no social pooling is taken into account. Therefore, here each pedestrian is not influenced by the surrounding people, and the relationship between the tracklets and the vislets in the prediction can be observed without any confounding factor. 
%These figures show different types of trajectories, each one equipped with its own vislets, here represented by the tip of the arrows: the blue one, which represents the routing input sequence given to the MX-LSTM. The green one is the ground-truth that has to be predicted. The yellow one is the prediction by MX-LSTM. The magenta one (left column) has been obtained by enforcing the vislets of the routing input sequence to point north (w.r.t. the image plane). The black one (center column) is the same as the magenta one, but pointing north. The red one (right column) has randomly placed vislets. The rationale of these last three types of sequences is to evaluate whether a different head pose behavior could trigger a diverse trajectory prediction. 
Fig.~\ref{fig:Qualitative}b) first row shows three situations in which the vislets of the observation sequence are artificially made pointing north (orange arrows), resulting not aligned with the trajectory. In this case the Individual MX-LSTM predicts a decelerating trajectory drifting toward north (magenta trajectory and vislets), especially in the second and third pictures.  If the observation has the legit vislets (green arrows, barely visible since they are aligned with the trajectory), the resulting trajectory (yellow trajectory and vislets) has a different behavior, closer to the GT (green trajectory and vislets). The second row is similar, with the observation vislets made pointing to south. The prediction with the modified vislets is in black. The only difference is in the bottom left picture: here the observation vislets pointing south are in accord with the movement, so that the resulting predicted trajectory is not decelerating as in the other cases, but accelerating toward south.



%(first column) and south (second column) do have a role in the trajectory prediction, being the related trajectories drifting themselves toward north and south. Interestingly, there is a general deceleration: this is the type of dynamics that happens when a person, while walking, turn his head to an object of interest, and changes direction slowing down to better look at it. Notably, all the vislets points have a distance which is somewhat constant (similar to $r$): this indicates that the LSTM has also captured the (artificial) distance between tracklet and vislet points. The unlikely vislet sequence (the red one, right column) lets the system predicts a fast trajectory with the vislets diverging from the trajectory. 

%Fig.~\ref{fig:Qualitative} second row
%30 1351  
%shows a %
%-->211359 - 563047
%similar behavior, going left to right: the purple sequence decelerate a little and goes north, the black one goes south.  

%Fig.~\ref{fig:Qualitative} third row 
%211239 
%shows that, for the individual going south, enforcing the head pose look north slows down dramatically the sequence, while looking south let the individual continue to go in that direction, while the correct trajectory was drifting left.




%%5935 4063 5215















\iffalse
\begin{table*}[t]
  \centering
  \vspace{10em}
  \caption{MAD -- Complete table: filled by Irtiza}
  \label{xx-}
  \scalebox{.88}{
  \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
    \hline
    Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
    \hline
    Zara01    &2.74  &2.88  &0.90  &0.89  &0.58  &0.63  &0.68  &0.66  &0.69 &0.63 &0.60 &0.60 \\
    \hline
    Zara02    &2.23  &2.32  &1.1  &0.89  &1.2  &0.72  &0.63  &0.48  &0.43 &0.36 &0.41 &0.35  \\
    \hline
    UCY        &2.49  &2.57  &0.67  &0.54  &0.84  &0.53  &0.62  &0.60  &0.58 &0.51 &0.54 &0.49  \\
    \hline
    TownCentre &  &  &4.62  &1.96  &2.67  &2.09  &1.96  &1.7  &1.9 &1.7 &1.4 &1.15  \\
    \hline \hline
    TownCentre (real HPE) &--  & --  &--  &2.08  &--  &2.18  &--  &1.7  &-- &1.7 &1.44 &1.2  \\
    \hline
  \end{tabular}
  }
  \caption{FAD -- Complete table: filled by Irtiza}
  \label{xx-}
  \scalebox{.88}{
  \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
    \hline
    Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
    \hline
    Zara01    &5.55  &5.55  &1.85  &1.81  &1.28  &1.37  &1.53  &1.51  &1.5 &1.40 &1.51 &1.31  \\
    \hline
    Zara02    &4.35  &4.35  &2.15  &1.90  &2.69  &1.56  &1.43  &1.06  &1.0 &0.84 &1.00 &0.79  \\
    \hline
    UCY        &4.66  &4.62  &1.39  &1.15  &1.92  &1.16  &1.40  &1.36  &1.27 &1.15 &1.23 &1.12  \\
    \hline
    TownCentre &  &  &8.26  &3.96  &5.15  &4.0  &3.96  &3.6  &4.2 &3.4 &2.9 &2.3  \\
    \hline \hline
    TownCentre (real HPE) &--  &--  &--  &4.12  &--  &4.2  &--  &3.6  &-- &3.4 &3.0 &2.36  \\
    \hline
  \end{tabular}
  }
\end{table*}







\fs{TO DO:
\begin{itemize}
    \item show the qualitative sequences in the text and show the distributions of LSTM, vislet LSTM (original data) and the distribution of the vislets
    \item 
\end{itemize}}
\fi


==> sections/experiments_v2.tex <==
\section{Experiments}
\label{sec:experiments}

% I believe this Section 5 preamble needs a bit of rewriting:
%   - intro of datasets
%   - intro of comparison to state of the art
%   - intro of ablation studies
%   - intro of qualitative results



We perform both qualitative and quantitative evaluations of our approach. For our experiments, we consider two public datasets for comparing with recent works. In addition, we provide an ablation study to show the contribution of the different MX-LSTM parts. On a further study, we consider whether ground-truth head pose information can be substituted by more accessible proxies, like step directions or simple head pose estimations (from a detector). On a qualitative evaluation, we provide visual proof of the interplay between tracklets and vislets that the MX-LSTM has learnt.

Next, we present in detail the analysis of our approach with respect to different time horizons, discussing how the different approaches perform in short and long term forecasting. It is illustrated how head pose plays a pivotal role for the long term forecasting. Finally, we introduce the first results on head pose forecasting.  

%% introduction
% The experiments are quantitative and qualitative. The former evaluate MX-LSTM and some variants on 4 datasets (the 3 UCY sequences Zara01, Zara02 and UCY~\cite{lerner2007crowds}, and the Town Centre dataset~\cite{benfold2011stable}); all the sequences have ground truth head poses, while on the Town Centre we manually added ground truth head poses and head poses estimated by~\cite{}. In all the cases,  the head poses are expressed as pan angles over the 360 circle. Comparative approaches are: Social Force model (SF)~\cite{}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, and Social LSTM (S-LSTM)~\cite{alahi2016cvpr}; in addition we use a vanilla LSTM model as baseline, removing the social pooling from the S-LSTM.
%\vspace{-0.1cm}

\subsection{Implementation details}
\label{sec:impl}

We implemented the MX-LSTM model and all models of the ablation study in Tensorflow. All models have been trained with learning rate of 0.005 along with the RMS-prop optimizer. We set the embedding dimension for spatial coordinates and vislets to 64 and the hidden state dimension is D = 128. We compute the social pooling on a grid of $32\times 32$ cells \eqref{eq:social}
%The grid for social pooling (Eq.~\eqref{eq:social}) has $N_o\times N_o$ cells with $N_o=32$.
The view frustum aperture angle has been cross-validated on the training partition of the TownCentre and kept fixed for the remaining trials ($\gamma=40^{\circ}$), while the depth $d$ is simply bounded by the social pooling grid. Training and testing has been accomplished with a GPU NVIDIA GTX-1080 for all evaluations.
%The MX-LSTM was trained on a single GPU with Tensorflow~\cite{abadi2016tensorflow} implementation. 



\subsection{Evaluation Protocol}
\label{sec:evaluation}
% Put here:
%  - datasets
%  - protocol
%  - metrics

We report experiments on two public datasets, namely \emph{UCY}~\cite{lerner2007crowds} and \emph{TownCentre}~\cite{benfold2011stable} datasets. The UCY dataset is composed of three sequences (\emph{Zara01}, \emph{Zara02}, and \emph{UCY}), taken in public spaces from top-view. In Table~\ref{tab:stat}, the statistics for each dataset are compared. For all sequences, manual annotations of people position and head pose is provided.
However, the TownCentre dataset has originally contained only pedestrian locations as ground-truth; we manually annotated the head pose for this sequence, which we already made public.

\begin{table}[]
\caption{Dataset Statistics}
 \label{tab:stat}
\begin{tabular}{|l|l|l|l|l|}
\hline
Dataset    & No. of  frames & No. of ped. & ped. per frame & avg traj. \\ \hline
Zara01     & 8,670          & 148         & 6              & 339       \\ \hline
Zara02     & 10.513         & 204         & 9              & 467       \\ \hline
UCY        & 5,405          & 434         & 32             & 404       \\ \hline
TownCentre & 4,500          & 230         & 16             & 310       \\ \hline
\end{tabular}
\end{table}

The evaluation protocol follows the standard procedure for trajectory forecasting that is used in the literature~\cite{pellegrini2009iccv,alahi2016cvpr}. We first downsampled the videos at 0.4fps, then we observe tracklets and vislets for 8 frames, and we predict both locations and head poses for the following 12 time steps.  The observation period is $3.2s$ and the forecasting horizon is $4.8s$. 
Experiments with different time horizons are reported in the ablation study (Sec.~\ref{sec:ablation}). According to the standard protocol, we used annotations during the observation period. Since we use additional information with respect to most of the related approaches (i.e. head poses), we perform an evaluation with the output of a real head pose estimator as well (Sec.~\ref{sec:ablation}). 

For the three UCY sequences we train three models, where we use two sequences for training and the remaining for testing. For the TownCentre dataset, the model has been trained and tested on the provided data splits.

Regarding the evaluation metrics of the trajectory forecasting, we consider the \emph{Mean Average Displacement} (MAD) error, \textit{i.e.} the average euclidean distance between all the predicted and ground-truth pedestrian locations. The \emph{Final Average Displacement} (FAD) error, \textit{i.e.} the euclidean distance between the last predicted location of each trajectory and the corresponding manually annotated point, is employed as well. Lastly, we evaluate the performance of the head pose predictions in terms of mean angular error $e_{\alpha}$, which is the mean absolute difference between the estimated pose and the annotated ground truth.

% \label{sec:metrics}
% In all the cases, the head poses are expressed as pan angles over the 360$^\circ$. Trajectory forecasting methods are quantitively analyzed by Mean Average Displacement (MAD) error, average euclidean distance between predicted point and ground truth point. Furthermore, we also evaluate Final Average Displacement error as a measure of quality which is essentially euclidean distance between the last predicted point and corresponding ground truth point.   

% %\subsection{Datasets}\label{sec:datasets}
% \myparagraph{UCY dataset.}
% UCY dataset~\cite{lerner2007crowds} composed of three sequences namely Zara01, Zara02, and UCY.
% All the sequences have ground truth head poses.

% \myparagraph{TownCenter.}
% we manually annotated ground truth head poses on TownCenter. We make public all the annotations done on TownCenter




\subsection{Comparison with Related Work}
\label{sec:sota}

% \subsection{Quantitative results}

%% Oracle experiments

% \begin{table*}[t]
%   \centering
%   \caption{Mean and Final Average Displacement errors (in meters) for all the methods on all the datasets.}
%   \label{tab:res-oracle}
%   \begin{tabular}{|c|l|*{6}{C{.093\textwidth}|}}
%     \hline
%     Metric & Dataset    &  SF~\cite{yamaguchi2011cvpr}  &  LTA~\cite{pellegrini2009iccv}   &  Vanilla LSTM~\cite{alahi2016cvpr}  & Social LSTM~\cite{alahi2016cvpr} & MX-LSTM  & {\it MX-LSTM (real HPE)} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Mean Average Displacement} & Zara01 & 2.88 & 2.74 & 0.90 & 0.68 & {\bf 0.59} & {\it 0.66} \\
%     \cline{2-8}
%     & Zara02    & 2.32 & 2.23 & 1.09 & 0.63 & {\bf 0.35} & {\it 0.37} \\
%     \cline{2-8}
%     & UCY        & 2.57 & 2.49 & 0.67 & 0.62 & {\bf 0.49} & {\it 0.55} \\
%     \cline{2-8}
%     & TownCentre &9.35 &9.14   & 4.62 & 1.96 & {\bf 1.15} & {\it 1.21} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 1.21} \\
%     \hline \hline
%     \multirow{5}{.14\textwidth}{\centering Final Average Displacement} & Zara01 & 5.55 & 5.55 & 1.85 & 1.53 & {\bf 1.31} & {\it 1.43} \\
%     \cline{2-8}
%     & Zara02    &  4.35 &  4.35 & 2.15 & 1.43 & {\bf 0.79} & {\it 0.82} \\
%     \cline{2-8}
%     & UCY        &  4.62 &  4.66 & 1.39 & 1.40 & {\bf 1.12} & {\it1.20 } \\
%     \cline{2-8}
%     & TownCentre & 16.01 & 16.08 & 8.26 & 3.96 & {\bf 2.30} & {\it 2.38} \\
%     % \cline{2-7}
%     % & {\it TownCentre (real HPE)} & {\it --} & {\it --} & {\it --} & {\it --} & {\it 2.38} \\
%     \hline
%   \end{tabular}
% \end{table*}

%\subsection{Quantitative results}\label{sec:quantitative}\vspace{-0.1cm}
We compare our model with one baseline, i.e. a standard LSTM model that only accounts for pedestrian positions (Vanilla LSTM), and four state-of-the-art approaches: Social Force model (SF)~\cite{yamaguchi2011cvpr}, Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}, Social LSTM (S-LSTM)~\cite{alahi2016cvpr} and Social GAN~\cite{SocialGAN18}.

Note that the Social GAN~\cite{SocialGAN18} requires ground-truth trajectories during the prediction interval: At test time, the Social GAN~\cite{SocialGAN18} model predicts 20 trajectories and uses the $L_2$ distance w.r.t the ground-truth trajectory to select the best one. Although this protocol makes the comparison with our approach unfair, we include it in the results for the sake of completeness. 
% This advantage is visible in the most linear dataset Zara01, where Social GAN~\cite{SocialGAN18} scores better than the proposed approach.
% For this reason, we do not consider this method as a fair comparison, and in the following of the discussion we will only refer to the other methods. \fs{this part is a bit tricky: I would put the Social GAN results in italic in Table 1 and clearly state that we only report results for the sake of completeness but we do not discuss their scores. I'd like to hear an opinion from all of you guys about this point.}
%Regarding the model parameters, the social pooling grid (Eq.~\eqref{eq:social}) has $N_o\times N_o$ cells with $N_o=32$. The view frustum aperture angle has been cross-validated on the training partition of the Town Center and kept fixed for the remaining trials ($\gamma=40^{\circ}$), while the depth $d$ is simply bounded by the social pooling grid. 

%The trajectory prediction performance is evaluated based on the Mean Average Displacement (MAD) error (euclidean distance between predicted and GT points, averaged over the sequence) and the Final Average Displacement (FAD) error (distance between the last predicted point and the corresponding GT point)~\cite{pellegrini2009iccv}.




\input{sections/table_stateoftheart_comparison}

Comparative results are reported in Table~\ref{tab:res-oracle}.
The MX-LSTM outperforms the state-of-the-art methods in all the sequences and with both metrics, with an average improvement of 23.3\% over the best performing competitors. The highest relative gain is achieved in the UCY sequence and TownCentre dataset, where complex non-linear paths are mostly caused by standing conversational groups and people that walk close to them, avoiding collisions.
People slowing down and looking at the window shops pose another challenge.
As shown in \figref{fig:angles}, slow moving and interacting pedestrians cause troubles to the competing methods, while MX-LSTM clearly overcomes such shortcomings denoting a better model.
% Note that the Social GAN~\cite{SocialGAN18} is the only method that uses ground-truth trajectories during prediction interval. At testing time, the Social GAN~\cite{SocialGAN18} model predicts 20 trajectories and uses the $L_2$ distance with the ground truth trajectory to pick the best one, which brings an intrinsic contradiction. This advantage is visible in the most linear dataset Zara01, where Social GAN~\cite{SocialGAN18} scores better than the proposed approach.
% For this reason, we do not consider this method as a fair comparison and in the following of the discussion we will only refer to the other methods. \fs{this part is a bit tricky: I would put the Social GAN results in italic in Table 1 and clearly state that we only report results for the sake of completeness but we do not discuss their scores. I'd like to hear an opinion from all of you guys about this point.}
%Qualitative evaluation follows in Sec.~\ref{sec:qualitative}.

Note that the evaluated methods rely on different input data: SF and LTA require the destination point of each individual, while SF requires social groups annotations. 


\subsubsection{Effect of head pose estimator}
\label{sec:exp-hpe}

MX-LSTM requires the head pose of each individual in each frame during the observation period, that is a relatively high amount of additional date to be provided; nevertheless, these information can be generated by a head pose estimator.
This motivates our next experiment: we automatically estimate the head bounding box given the feet positions on the floor plane, assuming an average person being $1.80$m tall. Then, we apply the head pose estimator of~\cite{hasan2017tiny} that provides continuous angles for the pan orientation. These data are then used as input to our approach (``MX-LSTM-HPE'' in Table~\ref{tab:res-oracle}. The use of a head pose estimator instead of manual annotations produces a drop in performances of less than 9\%, still beating the competitors in all the sequences, demonstrating that MX-LSTM does not suffer from small errors in the input head pose.
%\fs{I thought we used your ICIP estimator here?!?!}  
%As shown by the scores in Table~\ref{tab:res-oracle}, 
%These results demonstrate that MX-LSTM-HPE does not suffer from small errors in the input head pose, with an average drop in performances of only 5\% with respect with the manually annotated head poses during the observation period. In addition, MX-LSTM-HPE is still setting the state-of-the-art, even with noisy head poses at observation time.

But how accurate should the head pose estimation be for the MX-LSTM model to have convincing performances, i.e. to beat the state of the art? We answer this question by corrupting the annotated head poses with additive Gaussian noise $\sim\mathcal{N}(\alpha_t,\hat{\sigma})$, where $\alpha_t$ is the correct head pose and $\hat{\sigma}$ the standard deviation. MX-LSTM-HPE outperforms Social-LSTM up to a noise of $\hat{\sigma}=24^{\circ}$.

% Results are reported in ... (Table/Figure?)
% \fs{we should have a table or a plot for this experiment, otherwise I would rather remove it.}


\subsection{Ablation Study}
\label{sec:ablation}

Aside with the models in the literature, we investigate three variations of the MX-LSTM to capture the net contributions of the different parts that characterize our approach.

\subsubsection{Variants of MX-LSTM}
\label{sec:Variants}
\noindent\textbf{Block-Diagonal MX-LSTM (BD-MX-LSTM)}: This studies the importance of estimating full covariances to understand the interplay between tracklets and vislets, rather than modelling each of them as a separate probability distribution.  
%
%enforcing the LSTM to jointly studying the separated information streams, tracklets and vislets, through the full covariance. 
Essentially, instead of learning the $4\times4$ full covariance matrix $\mathbf{\Sigma}$, BD-MX-LSTM estimates two separate bidimensional covariances $\mathbf{\Sigma}_x$ and $\mathbf{\Sigma}_a$ for the trajectory and the vislet modeling, thus neglecting the cross-stream covariance. Each $2\times2$ covariance is estimated employing two variances $\sigma_1, \sigma_2$ and a correlation terms $\rho$ as presented in~\cite{graves2013generating}. % Eq.(24) and (25).
% \emph{The equations that differ w.r.t. MX-LSTM will be given as supplemental material.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
The equations that differ from the proposed MX-LSTM are Eq.~\eqref{eq:LLog} and Eq.~\eqref{eq:params}, which become:
\begin{eqnarray}
L^i(\mathbf{W}_{x},\mathbf{W}_{a},\mathbf{W}_H,\mathbf{W}_{\text{LSTM}},\mathbf{W}_{o}) &=&\nonumber\\  -\sum_{T_{obs}+1}^{T_{pred}}log\left( P([\mathbf{x}^{(i)}_t]^T|\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t \right)+\!\!\\\nonumber
log\left(P([\mathbf{a}^{(i)}_t]^T|\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t\right)
\end{eqnarray}
where $\bo{\mu}^{(x,i)}_t=[{}_x\mu^{(x,i)}_t,{}_y\mu^{(x,i)}_t]$ and the same apply for the variance vector;
\begin{equation}
[\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t,\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t]^T \!=\! \mathbf{W}_o \mathbf{h}^{(i)}_{t-1}\label{eq:params}
\end{equation}
%\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \fs{double check these equations!!!}

\noindent\textbf{NoFrustum MX-LSTM}: this variant reduces MX-LSTM to the social pooling of~\cite{alahi2016cvpr}, i.e.\ pooling for hidden states $\{\mathbf{h}^{j}_t\}$ from the entire area around each individual. NoFrustum MX-LSTM neglects the visual frustum of attention and does not select the people to pool from based on it. Also people behind the person would therefore influence the next step forecasting.

\noindent\textbf{Individual MX-LSTM}: in this case, no social pooling is taken into account. In more detail, the embedding operation of Eq.~\eqref{eq:pooling} is removed, and the weight matrix $\mathbf{W}_H$ vanishes. In practice, this variant learns independent models for each person, each one considering the tracklet and vislet points.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Error metric (MAD). 12, 14…32 corresponds to horizon intervals for prediction. Observation interval is kept constant (8 frames). Smaller Observation Interval, H=12. larger Observation=16 Interval larger prediction interval.}
% \label{table:table1}
% \resizebox{.999\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|}
% \cline{1-8} \cline{10-13} \cline{15-19}
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{\underline{H = 12}} & \textbf{H = 16} & \textbf{H = 20} & \textbf{H = 24} & \textbf{H = 28} & \textbf{H = 32} &  & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} &  & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.90            & 1.21            & 1.70            & 2.30            & 3.07            & 4.11            &  & 1.62             & 0.90             & 0.90             & 0.90              &  & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.72            & 1.05            & 1.44            & 1.85            & 2.47            & 3.14            &  & 1.43             & 0.79             & 0.72             & 0.60              &  & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.68            & 1.00            & 1.43            & 1.94            & 2.35            & 2.85            &  & \textbf{0.89}             & 0.69             & 0.68             & 0.68              &  & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.59}   & \textbf{0.87}   & \textbf{1.21}   & \textbf{1.55}   & \textbf{1.92}   & \textbf{2.40}   &  & 0.96    & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     &  & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 1.09            & 1.62            & 2.19            & 2.75            & 3.31            & 3.86            &  & 1.65             & 1.17             & 1.09             & 0.99              &  & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.63            & 1.09            & 1.43            & 1.83            & 2.25            & 2.67            &  & 1.35             & 0.84             & 0.63             & 0.62              &  & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.63            & 0.90            & 1.24            & 1.59            & 2.00            & 2.41            &  & 1.13             & 0.74             & 0.63             & 0.63              &  & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.35}   & \textbf{0.53}   & \textbf{0.71}   & \textbf{0.90}   & \textbf{1.16}   & \textbf{1.40}   &  & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     &  & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \multirow{4}{*}{\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.67            & 0.90            & 1.19            & 1.52            & 1.87            & 2.24            &  & 0.82             & 0.65             & 0.67             & 0.63              &  & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.53            & 0.77            & 1.01            & 1.27            & 1.53            & 1.83            &  & 0.88             & 0.59             & 0.53             & 0.52              &  & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.62            & 0.90            & 1.08            & 1.36            & 1.66            & 1.99            &  & 0.71             & 0.63             & 0.62             & 0.60              &  & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-8} \cline{10-13} \cline{15-19} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.49}   & \textbf{0.70}   & \textbf{0.95}   & \textbf{1.22}   & \textbf{1.50}   & \textbf{1.80}   &  & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     &  & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \cline{1-8} \cline{10-13} \cline{15-19} 
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Error metric (MAD). 12, 14…32 corresponds to horizon intervals for prediction. Observation interval is kept constant (8 frames). Smaller Observation Interval, H=12. larger Observation=16 Interval larger prediction interval.}
% \label{table:table1}
% \resizebox{.999\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c!{\vrule width2pt}c|c|c|c!{\vrule width2pt}c|c|c|c|c|}
% \hline
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{\underline{H = 12}} & \textbf{H = 16} & \textbf{H = 20} & \textbf{H = 24} & \textbf{H = 28} & \textbf{H = 32} & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \hline
% \multirow{4}{*}{\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.90            & 1.21            & 1.70            & 2.30            & 3.07            & 4.11            & 1.62             & 0.90             & 0.90             & 0.90              & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.72            & 1.05            & 1.44            & 1.85            & 2.47            & 3.14            & 1.43             & 0.79             & 0.72             & 0.60              & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.68            & 1.00            & 1.43            & 1.94            & 2.35            & 2.85            & 0.89             & 0.69             & 0.68             & 0.68              & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.59}   & \textbf{0.87}   & \textbf{1.21}   & \textbf{1.55}   & \textbf{1.92}   & \textbf{2.40}   & \textbf{0.96}    & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \hline
% \multirow{4}{*}{\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 1.09            & 1.62            & 2.19            & 2.75            & 3.31            & 3.86            & 1.65             & 1.17             & 1.09             & 0.99              & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.63            & 1.09            & 1.43            & 1.83            & 2.25            & 2.67            & 1.35             & 0.84             & 0.63             & 0.62              & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.63            & 0.90            & 1.24            & 1.59            & 2.00            & 2.41            & 1.13             & 0.74             & 0.63             & 0.63              & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.35}   & \textbf{0.53}   & \textbf{0.71}   & \textbf{0.90}   & \textbf{1.16}   & \textbf{1.40}   & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \hline
% \multirow{4}{*}{\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ LSTM\end{tabular}}       & 0.67            & 0.90            & 1.19            & 1.52            & 1.87            & 2.24            & 0.82             & 0.65             & 0.67             & 0.63              & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ MX-LSTM\end{tabular}} & 0.53            & 0.77            & 1.01            & 1.27            & 1.53            & 1.83            & 0.88             & 0.59             & 0.53             & 0.52              & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-17} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\\ LSTM\end{tabular}}        & 0.62            & 0.90            & 1.08            & 1.36            & 1.66            & 1.99            & 0.71             & 0.63             & 0.62             & 0.60              & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-17} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.49}   & \textbf{0.70}   & \textbf{0.95}   & \textbf{1.22}   & \textbf{1.50}   & \textbf{1.80}   & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \hline
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
%\renewcommand{\arraystretch}{2}

% \begin{table}[t]
%   \centering
%   \caption{Mean Average Displacement (MAD) error when changing the forecasting horizon. Observation interval is kept constant at 8 frames.}
%   \label{table:table1Ab}
%   \resizebox{\linewidth}{!}{
%     %\begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \begin{tabular}{|c|c *{6}{|C{.046\textwidth}}|}
%     \hline
%     \textbf{Dataset} & \textbf{Method} & \textbf{\underline{H = 12}} & \textbf{H = 16} & \textbf{H = 20} & \textbf{H = 24} & \textbf{H = 28} & \textbf{H = 32} \\ 
%     \hline \hline
%     \multirow{4}{*}{\textbf{Zara 01}} & 
%     Vanilla LSTM & 0.90 & 1.21 & 1.70 & 2.30 & 3.07 & 4.11 \\
%     \cline{2-8} 
%     & Individual MX-LSTM & 0.72 & 1.05 & 1.44 & 1.85 & 2.47 & 3.14 \\
%     \cline{2-8} 
%     & Social LSTM & 0.68 & 1.00 & 1.43 & 1.94 & 2.35 & 2.85 \\
%     \cline{2-8} 
%     & MX-LSTM & \textbf{0.59} & \textbf{0.87} & \textbf{1.21} & \textbf{1.55} & \textbf{1.92} & \textbf{2.40} \\ 
%     \hline \hline
%     \multirow{4}{*}{\textbf{Zara 02}} & 
%     Vanilla LSTM & 1.09 & 1.62 & 2.19 & 2.75 & 3.31 & 3.86 \\
%     \cline{2-8} 
%     & Individual MX-LSTM & 0.63 & 1.09 & 1.43 & 1.83 & 2.25 & 2.67 \\
%     \cline{2-8} 
%     & Social LSTM & 0.63 & 0.90 & 1.24 & 1.59 & 2.00 & 2.41 \\
%     \cline{2-8} 
%     & MX-LSTM & \textbf{0.35} & \textbf{0.53} & \textbf{0.71} & \textbf{0.90} & \textbf{1.16} & \textbf{1.40} \\
%     \hline \hline
%     \multirow{4}{*}{\textbf{UCY}} & 
%     Vanilla LSTM & 0.67 & 0.90 & 1.19 & 1.52 & 1.87 & 2.24 \\
%     \cline{2-8} 
%     & Individual MX-LSTM & 0.53 & 0.77 & 1.01 & 1.27 & 1.53 & 1.83 \\
%     \cline{2-8} 
%     & Social LSTM & 0.62 & 0.90 & 1.08 & 1.36 & 1.66 & 1.99 \\
%     \cline{2-8} 
%     & MX-LSTM & \textbf{0.49} & \textbf{0.70} & \textbf{0.95} & \textbf{1.22} & \textbf{1.50} & \textbf{1.80} \\
%     \hline
%     \end{tabular}
%   }
% \end{table}
% %\renewcommand{\arraystretch}{1}



% \renewcommand{\arraystretch}{2}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[!htb]
% \centering
% \caption{Smaller Observation Interval, H=12.}
% \label{table:table2Ab}
% \resizebox{.999\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{Obs = 1} & \textbf{Obs = 4} & \textbf{Obs = 8} & \textbf{\underline{Obs = 16}} \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.62             & 0.90             & 0.90             & 0.90              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 1.43             & 0.79             & 0.72             & 0.60              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & \textbf{0.89}    & 0.69             & 0.68             & 0.68              \\ \cline{2-6} 
%                                   & \textbf{MX-LSTM}                                                      & 0.96             & \textbf{0.64}    & \textbf{0.59}    & \textbf{0.59}     \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.65             & 1.17             & 1.09             & 0.99              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 1.35             & 0.84             & 0.63             & 0.62              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 1.13             & 0.74             & 0.63             & 0.63              \\ \cline{2-6} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.85}    & \textbf{0.48}    & \textbf{0.35}    & \textbf{0.33}     \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 0.82             & 0.65             & 0.67             & 0.63              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.88             & 0.59             & 0.53             & 0.52              \\ \cline{2-6} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.71             & 0.63             & 0.62             & 0.60              \\ \cline{2-6} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.62}    & \textbf{0.49}    & \textbf{0.49}    & \textbf{0.48}     \\ \hline
% \end{tabular}}
% \end{table}
% \renewcommand{\arraystretch}{1}

% \renewcommand{\arraystretch}{2}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[!htb]
% \centering
% \caption{larger Observation=16 Interval larger prediction interval.}
% \label{table:table3Ab}
% \resizebox{.999\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset}                  & \textbf{Method}                                                       & \textbf{Pred = 16} & \textbf{Pred = 20} & \textbf{Pred = 24} & \textbf{Pred = 28} & \textbf{Pred = 32} \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{Zara 01}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.25               & 1.27               & 1.78               & 2.39               & 3.09               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.90               & 1.266              & 1.6401             & 2.01               & 2.57               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 1.0568             & 1.46               & 1.88               & 2.37               & 3.00               \\ \cline{2-7} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.8840}    & \textbf{1.19}      & \textbf{1.5712}    & \textbf{1.93}      & \textbf{2.32}      \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{Zara 02}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.315              & 1.872              & 2.50               & 3.19               & 3.87               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.95               & 1.28               & 1.65               & 2.048              & 2.42               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.8845             & 1.24               & 1.61               & 2.05               & 2.53               \\ \cline{2-7} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.49}      & \textbf{0.67}      & \textbf{0.87}      & \textbf{1.112}     & \textbf{1.3517}    \\ \hline
% \multirow{4}{*}{\vspace{-35pt}\textbf{UCY}}     & \textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\vspace{-7pt}\\ LSTM\end{tabular}}       & 1.02               & 1.42               & 1.87               & 2.37               & 2.92               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\vspace{-7pt}\\ MX-LSTM\end{tabular}} & 0.72               & 1.01               & 1.4                & 1.50               & 1.90               \\ \cline{2-7} 
%                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Social\vspace{-7pt}\\ LSTM\end{tabular}}        & 0.801              & 1.063              & 1.34               & 1.67               & 2.21               \\ \cline{2-7} 
%                                   & \textbf{MX-LSTM}                                                      & \textbf{0.71}      & \textbf{0.95}      & \textbf{1.2}       & \textbf{1.46}      & \textbf{1.8017}    \\ \hline
% \end{tabular}}
% \end{table}
% \renewcommand{\arraystretch}{1}

\renewcommand{\arraystretch}{2}
\begin{table}[t]
  \centering
  \caption{larger Observation=16 Interval larger prediction interval.}
  \label{table:table3Ab}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|c *{5}{|C{.075\textwidth}}|}
    \hline
    Dataset & Prediction interval & Vanilla LSTM & Social LSTM & MX-LSTM & Individual MX-LSTM \\
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 01}} & 
    \textbf{Pred = 16} & 1.25 & 1.05 & {\bf 0.88} & 0.90 \\
    \cline{2-6}
    & \textbf{Pred = 20} & 1.27 & 1.46 & {\bf 1.19} & 1.26 \\
    \cline{2-6}
    & \textbf{Pred = 24} & 1.78 & 1.88 & {\bf 1.57} & 1.64 \\
    \cline{2-6}
    & \textbf{Pred = 28} & 2.39 &2.37 &{\bf 1.93} & 2.01 \\
    \cline{2-6}
    & \textbf{Pred = 32} & 3.09 & 3.00 & {\bf 2.32} & 2.57 \\

    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 02}} & 
    \textbf{Pred = 16} & 1.31 & 0.88 & {\bf 0.49} & 0.95 \\
    \cline{2-6}
    & \textbf{Pred = 20} & 1.87 & 1.24 & {\bf 0.67} & 1.28 \\
    \cline{2-6}
    & \textbf{Pred = 24} & 2.50 & 1.61 & {\bf 0.87} & 1.65 \\
    \cline{2-6}
    & \textbf{Pred = 28} &3.19 &2.05 &{\bf 1.11} & 2.04 \\
    \cline{2-6}
    & \textbf{Pred = 32} & 3.87 & 2.53 & {\bf 1.35} & 2.42 \\

    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{UCY}} & 
    \textbf{Pred = 16} & 1.02 & 0.80 & {\bf 0.71} & 0.72 \\
    \cline{2-6}
    & \textbf{Pred = 20} & 1.42 & 1.06 & {\bf 0.95} & 1.01 \\
    \cline{2-6}
    & \textbf{Pred = 24} & 1.87 & 1.34 & {\bf 1.2} & 1.40 \\
    \cline{2-6}
    & \textbf{Pred = 28} &2.37 &1.67 &{\bf 1.46} & 1.50 \\
    \cline{2-6}
    & \textbf{Pred = 32} & 2.92 & 2.21 & {\bf 1.80} & 1.90 \\
     \hline
    \end{tabular}
  }
\end{table}
\renewcommand{\arraystretch}{1}

\vspace{1em}
The last three columns of Table~\ref{tab:res-oracle} report numerical results for the three MX-LSTM variants. The main facts that emerge are: 1) the highest variations are with the Zara02 sequence, where MX-LSTM doubles the performances of the worst approach (Individual MX-LSTM); 2) the worst performing is in general Individual MX-LSTM, showing that social reasoning is indeed needed; 3) social reasoning is systematically improved with the help of the vislet-based view-frustum; 4) full covariance estimation has a role in pushing down the error which is already small with the adoption of vislets.

% \fs{expand and smooth these paragraph.}

Summarizing the results so far, having vislets as input allows to definitely increase the trajectory forecasting performance, even if vislets are estimated with a certain amount of noise. Vislets should be used to understand social interactions with social pooling, by building a view frustum that tells which are the people currently observed by each individual. All of these features are effectively and efficiently implemented within MX-LSTM. Note in fact that the training time is not affected by whether social pooling is included or not.

Again, although the complete method always outperforms all the competitors, the highest improvement is on the TownCentre sequence. In our opinion this is due to the different level of complexity in the data, indeed most of the trajectories in UCY sequences are relatively linear, with poor social interactions, while in TownCentre there are many interactions, such as forming and splitting groups and crossing trajectories.
For the same reason, this is the dataset where the introduction of the view frustum in the pooling of social interactions gives the highest benefits. By contrast, in all other sequences but Zara01, decoupling the covariance matrix into a block diagonal matrix neglecting the interplay of position and gaze (BD-MX-LSTM) leads to a sensitive increase in the prediction error; this proves the tight relation between the head orientation and the motion of an individual.


\subsubsection{Head Pose Forecasting}\vspace{-0.1cm}
Our MX-LSTM model also provides a forecast of the head pose of each individual at each frame, for the first time. We evaluate the performances of this estimation in terms of mean angular error $e_{\alpha}$, i.e.\ the mean absolute difference between the estimated pose (angle $\alpha_{t,\cdot}$ in \figref{fig:explanations}c) and the annotated ground truth.
%is equal to the pose plausibility error, with $\alpha_{t,\cdot}$ instead of $\omega_{t,\cdot}$.
$e_{\alpha}$ expresses how much the direction in which an individual is looking at a particular time instant is different from the true one. This error measure is independent from the error in the predicted position. In other words, $e_{\alpha}$ measures the error in the gaze forecasting.
%of interest, especially in coincidence with a low MAD, as it is in general in our experiments.   

% \begin{table}[t!]
%   \centering
%   \caption{Pose plausibility error ($e_{\text{pp}}$) and angular error ($e_{\alpha}$) for the MX-LSTM model on all the datasets.}
%   \label{tab:res-angle}
%   \begin{tabular}{|l|*{2}{C{.1\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     TownCentre &  23.30  &  26.48  \\
%     \hline
%   \end{tabular}
% \end{table}

%\renewcommand{\arraystretch}{2}
\begin{table}[t!]
  \centering
%  \small
  \caption{Mean angular error (in degrees) for the state-of-the-art head pose estimator~\cite{hasan2017tiny}, and our model fed with manual annotations (MX-LSTM) and estimated values (MX-LSTM-HPE).}
  \label{tab:res-angle}
%  \resizebox{\linewidth}{!}{
%  \begin{tabular}{|l|c|c|c|c|}
%   \begin{tabular}{|l *{4}{|C{.075\textwidth}}|}
%     \hline
%     Metric                 &  Zara01  &  Zara02  &   UCY   &  Town Centre \\
%     \hline
%     HPE~\cite{lee2015fast} &  14.29   &   20.02  &  19.90  &   25.08    \\   
%     \hline
%     MX-LSTM                &  12.98   &   20.55  &  21.36  &   26.48    \\
%     \hline
%     MX-LSTM-HPE            &  17.69   &   21.92  &  24.37  &   28.55  \\
%     \hline
%   \end{tabular}
%  }
  \resizebox{\linewidth}{!}{
  \begin{tabular}{|l *{4}{|C{.11\textwidth}}|}
    \hline
    Metric         & HPE~\cite{hasan2017tiny} & MX-LSTM & MX-LSTM-HPE \\
    \hline
    Zara01         & 14.29 & 12.98 & 17.69 \\   
    \hline
    Zara02         & 20.02 & 20.55 & 21.92 \\
    \hline
    UCY            & 19.90 & 21.36 & 24.37 \\
    \hline
    TownCentre     & 25.08 & 26.48 & 28.55 \\
    \hline
  \end{tabular}
  }
\end{table}
\renewcommand{\arraystretch}{1}





% \begin{table}[t!]
%   \centering
%   \begin{minipage}[t]{.39\columnwidth}
%     \centering
%     \caption{Head pose estimation errors for MX-LSTM on all the datasets (in degrees).}
%     \label{tab:res-angle}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{|l|*{2}{C{.25\textwidth}|}}
%     \hline
%     Dataset    &  $e_{\text{pp}}$  &  $e_{\alpha}$  \\
%     \hline
%     Zara01     &   9.62  &  12.98  \\
%     \hline
%     Zara02     &  33.93  &  20.55  \\
%     \hline
%     UCY        &  21.70  &  21.36  \\
%     \hline
%     Town Centre &  23.30  &  26.48  \\
%     \hline
%     \end{tabular}
%     }
%   \end{minipage}
%   \hspace{.02\linewidth}
%   \begin{minipage}[t]{.57\columnwidth}
%     \centering
%     \caption{Boh}
%     \label{fig:angle}
%     \includegraphics[width=\linewidth]{figure/supercool.pdf}
%   \end{minipage}
% \end{table}



Table~\ref{tab:res-angle} reports numerical results of the static head pose estimator~\cite{lee2015fast} (HPE), the proposed model fed with manually annotated head poses (MX-LSTM) and with the output of HPE (MX-LSTM-HPE) during the observation period.
In all the cases our forecast output is comparable with the one of HPE, but in our case we do not use appearance cues -- i.e. we do not look at the images at all.
In the case of Zara01, the MX-LSTM is even better that the static prediction, which highlights the forecasting power of our model. In our opinion, this is due to the fact that in this sequence trajectories are mostly linear and that people are walking fast, with their heads mostly aligned with the direction of motion. When providing the MX-LSTM model with the estimations during the observation period, the angular error increases, as expected, but the error remains limited.
%The low error achieved in Zara01 is probably related to the fact that this sequence is dominated people moving linearly and fast, thus the head orientation is usually aligned with the trajectory and the model can learn this behavior very easily.
%Zara02: more complicate, people are standing more in between of people moving fast (right Irtiza?) so big variety of disalignments, and you have the biggest errors
%Zara02 is a more challenging sequence, since there is a high number of standing group formations in the middle of the scene; these trajectories are very noisy, and as a consequence $e_{\text{pp}}$ increase.
%UCY: still group formations, but they are moving, so less disalignment and noise, numbers are in accord with this (Irtiza agree?)
%In UCY, the grouping formations are still present, but in this case they are moving, so noise is reduced and thus the disalignement between trajectory and head pose.



\subsubsection{Time Horizon Effect}
\label{sec:horizon}
% \todo{ Explain the bullet points and place all the relevant tables
% \begin{itemize}
%     \item We show that MX-LSTM is also more accurate in long term forecasting;
%     %the head pose, also given by a normal head pose estimator;\vspace{-5pt}
%     \item we illustrate that social LSTM degrades as we increase the prediction interval
%     \item We motivate that even with fewer observation interval the injection of head pose provides useful information in long term forecasting. 
%     \item We present ranking order remains same in all experiment.
% \end{itemize}
% }

\begin{table}[t]
  \centering
  \caption{Mean Average Displacement (MAD) error when changing the forecasting horizon. Observation interval is kept constant at 8 frames.}
  \label{table:table1Ab}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|c *{5}{|C{.075\textwidth}}|}
    \hline
    Dataset & Forecasting horizon & Vanilla LSTM & Social LSTM & MX-LSTM & Individual MX-LSTM \\
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 01}} & 
    \textbf{\underline{H = 12}} & 0.90 & 0.68 & {\bf 0.59} & 0.72 \\
    \cline{2-6}
    & \textbf{H = 16} & 1.21 & 1.00 & {\bf 0.87} & 1.05 \\
    \cline{2-6}
    & \textbf{H = 20} & 1.70 & 1.43 & {\bf 1.21} & 1.44 \\
    \cline{2-6}
    & \textbf{H = 24} & 2.30 & 1.94 & {\bf 1.55} & 1.85 \\
    \cline{2-6}
    & \textbf{H = 28} & 3.07 & 2.35 & {\bf 1.92} & 2.47 \\
    \cline{2-6}
    & \textbf{H = 32} & 4.11 & 2.85 & {\bf 2.40} & 3.14 \\ 
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 02}} & 
    \textbf{\underline{H = 12}} & 1.09 & 0.63 & {\bf 0.35} & 0.63 \\
    \cline{2-6}
    & \textbf{H = 16} & 1.62 & 0.90 & {\bf 0.53} & 1.09 \\
    \cline{2-6}
    & \textbf{H = 20} & 2.19 & 1.24 & {\bf 0.71} & 1.43 \\
    \cline{2-6}
    & \textbf{H = 24} & 2.75 & 1.59 & {\bf 0.90} & 1.83 \\
    \cline{2-6}
    & \textbf{H = 28} & 3.31 & 2.00 & {\bf 1.16} & 2.25 \\
    \cline{2-6}
    & \textbf{H = 32} & 3.86 & 2.41 & {\bf 1.40} & 2.67 \\ 
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{UCY}} & 
    \textbf{\underline{H = 12}} & 0.67 & 0.62 & {\bf 0.49} & 0.53 \\
    \cline{2-6}
    & \textbf{H = 16} & 0.90 & 0.90 & {\bf 0.70} & 0.77 \\
    \cline{2-6}
    & \textbf{H = 20} & 1.19 & 1.08 & {\bf 0.95} & 1.01 \\
    \cline{2-6}
    & \textbf{H = 24} & 1.52 & 1.36 & {\bf 1.22} & 1.27 \\
    \cline{2-6}
    & \textbf{H = 28} & 1.87 & 1.66 & {\bf 1.50} & 1.53 \\
    \cline{2-6}
    & \textbf{H = 32} & 2.24 & 1.99 & {\bf 1.80} & 1.83 \\ 
    % \hline \hline
    % \multirow{4}{*}{\vspace{-2.5em}\textbf{TownCentre}} & 
    % \textbf{\underline{H = 12}} & 4.62 & 1.96 & {\bf 1.15} & 2.09 \\
    % \cline{2-6}
    % & \textbf{H = 16} & & & & \\
    % \cline{2-6}
    % & \textbf{H = 20} & & & & \\
    % \cline{2-6}
    % & \textbf{H = 24} & & & & \\
    % \cline{2-6}
    % & \textbf{H = 28} & & & & \\
    % \cline{2-6}
    % & \textbf{H = 32} & & & & \\ 
    \hline
    \end{tabular}
  }
\end{table}

%\fs{Why don't we provide results for FAD and for TownCentre dataset? And how did we choose which methods to compare? We should be extremely clear in the text!}
% \fs{Say something about why we only consider Individual MX-LSTM whithin all the MX-LSTM versions.}

In order to understand how MX-LSTM performs for longer time horizons we conducted an experimental evaluation where we increment the prediction interval from 12 (standard evaluation protocol) to 32 frames with a step size of 4, keeping the observation interval fixed at 8 frames. We evaluated approaches on UCY, Zara01 and Zara02, since most trajectories on TownCenter last less than 24 frames.       
We use MAD to report the error.
% \fs{Say something about why we do not use FAD.}
As shown in Table~\ref{table:table1Ab}, MX-LSTM is well capable of handling longer time horizons. MX-LSTM outperforms all other approaches on all prediction interval, which demonstrates its robustness. 
Based on these results, we argue that reasoning on the head pose becomes even more important when forecastign in the longer term. Overall, the ranking is preserved and MX-LSTM remains the best performer.  


\begin{table}[t]
  \centering
  \caption{Mean Average Displacement (MAD) error when changing the observation period. Forecasting horizon is kept constant at 12 frames.}
  \label{table:table2Ab}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|c *{5}{|C{.075\textwidth}}|}
    \hline
    Dataset & Observation period & Vanilla LSTM & Social LSTM & MX-LSTM & Individual MX-LSTM \\
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 01}} & 
    \textbf{O = 1} & 1.62 & {\bf 0.89} & 0.96 & 1.43 \\
    \cline{2-6}
    & \textbf{O = 4} & 0.90 & 0.69 & {\bf 0.64} & 0.79 \\
    \cline{2-6}
    & \textbf{\underline{O = 8}} & 0.90 & 0.68 & {\bf 0.59} & 0.72 \\
    \cline{2-6}
    & \textbf{O = 12} &0.90 &0.68 &{\bf 0.59} & 0.68 \\
    \cline{2-6}
    & \textbf{O = 16} & 0.90 & 0.68 & {\bf 0.59} & 0.60 \\
    % \cline{2-6}
    % & \textbf{H = 28} & 3.07 & 2.35 & {\bf 1.92} & 2.47 \\
    % \cline{2-6}
    % & \textbf{H = 32} & 4.11 & 2.85 & {\bf 2.40} & 3.14 \\ 
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{Zara 02}} & 
    \textbf{O = 1} & 1.65 & 1.13 & {\bf 0.85} & 1.35 \\
    \cline{2-6}
    & \textbf{O = 4} & 1.17 & 0.74 & {\bf 0.48} & 0.84 \\
    \cline{2-6}
    & \textbf{\underline{O = 8}} & 1.09 & 0.63 & {\bf 0.35} & 0.63 \\
    \cline{2-6}
    & \textbf{O = 12} &1.01 &0.63 &{\bf 0.35} & 0.63 \\
    \cline{2-6}
    & \textbf{O = 16} & 0.99 & 0.63 & {\bf 0.33} & 0.62 \\
    % \cline{2-6}
    % & \textbf{H = 28} & 3.31 & 2.00 & {\bf 1.16} & 2.25 \\
    % \cline{2-6}
    % & \textbf{H = 32} & 3.86 & 2.41 & {\bf 1.40} & 2.67 \\ 
    \hline \hline
    \multirow{4}{*}{\vspace{-2.5em}\textbf{UCY}} & 
    \textbf{O = 1} & 0.82 & 0.71 & {\bf 0.62} & 0.88 \\
    \cline{2-6}
    & \textbf{O = 4} & 0.65 & 0.63 & {\bf 0.49} & 0.59 \\
    \cline{2-6}
    & \textbf{\underline{O = 8}} & 0.67 & 0.62 & {\bf 0.49} & 0.53 \\
    \cline{2-6}
    & \textbf{O = 12} &0.65 &0.60 &{\bf 0.48} & 0.52 \\
    \cline{2-6}
    & \textbf{O = 16} & 0.63 & 0.60 & {\bf 0.48} & 0.52 \\
    % \cline{2-6}
    % & \textbf{H = 28} & 1.87 & 1.66 & {\bf 1.50} & 1.53 \\
    % \cline{2-6}
    % & \textbf{H = 32} & 2.24 & 1.99 & {\bf 1.80} & 1.83 \\ 
    % \hline \hline
    % \multirow{4}{*}{\vspace{-2.5em}\textbf{TownCentre}} & 
    % \textbf{O = 1} & & & & \\
    % \cline{2-6}
    % & \textbf{O = 4} & & & & \\
    % \cline{2-6}
    % & \textbf{\underline{O = 8}} & 4.62 & 1.96 & {\bf 1.15} & 2.09 \\
    % \cline{2-6}
    % & \textbf{O = 12} & & & & \\
    % \cline{2-6}
    % & \textbf{O = 16} & & & & \\
    % % \cline{2-6}
    % % & \textbf{H = 28} & & & & \\
    % % \cline{2-6}
    % % & \textbf{H = 32} & & & & \\ 
     \hline
    \end{tabular}
  }
\end{table}


In order to understand how many frames are enough to learn a meaningful representation of the trajectory we varied the observation interval.
%
Table 5, reports numerical results of an experiment where we kept the forecasting horizon fixed at 12 frames, and varied the observation period form 1 to 16 frames with the step size of 4 frames.
An observation period of 1 frame means we try to predict trajectories based only on a static observation of the individual, with no previous history taken into account. Results prove that one frame is not enough for all the methods under analysis. Despite this, the ranking of different approaches is maintained throughout all the experiments, with the only exception of Zara01 sequence with O=1, where Social LSTM outperforms competitors.
Interestingly, a rapid drop in error of about 30\% is obtained by observing 4 frames instead of 1. Furthermore, 8 frames are enough for the approaches to learn the overall shape of the trajectory in order to predict for the next 12 frames, as the error drop from observing 8 frames to 16 frames is below 1\%.

Finally, in order to understand in more depth how different methods perform for long term forecasting, we kept the observation interval constant at 16 frames and test increasing forecasting horizons. Table~\ref{table:table3Ab}, further validates the fact that 8 frames are sufficient for the LSTM approach to learn the representation of the trajectory. MX-LSTM is still the best performer but the error drop from observing 8 to observing 16 frames is negligible in long term forecatsing as well. This effect also illustrates about the capacity of the LSTM based approach. At 8 frames, the performance already starts to saturate, therefore adding more information does not bring any new meaningful information to learn. This can bee seen as the performance bottle neck of all LSTM based approaches.

% \fs{honestly I do not understand this experiment and I don't find it convincing. This is just the same as Table~\ref{table:table1Ab} with a longer observation period. If we want to analyse the correlation between the observation period O and the forecasting horizon H this is not enough to me. On the other hand, I do not see this experiment as useful from the discussion above.}


\subsubsection{Substitute for Head Pose}\vspace{-0.1cm}
In this experiment, we analyzed the importance of the head pose and answered the question as to whether it may be substituted by more accessible proxies, such as step directions or simple head pose estimations. In more details,
we implemented a Pace-MX-LSTM, which uses ground truth step directions instead of the head pose. Table~\ref{table:step} illustrates that Having the step direction instead of the head pose represents a downgrade for MX-LSTM, since positional data are already contained in the tracklet and the step direction can be extracted from the previous two positions. In fact, Pace-MX-LSTM gives consistently worse results. 

Additionally, we implemented the MX-LSTM-HPE-Train and Test,
where the head pose training data is given by a detector~\cite{hasan2017tiny}. Performances (see Table~\ref{table:step}) are obviously worse than MX-LSTM-HPE (where only the test sequences consist of head pose estimations), especially on Zara02, where conversational groups make the head pose estimation noisy due to the many partial occlusions. Still MX-LSTM-HPE-Train
and Test remains comparable to prior state-of-the-art methods.






\vspace{-0.2cm}

\subsection{Qualitative Results}
\label{sec:qualitative}

    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/Qualitative8_theo.png}
		\caption{Qualitative results: a) MX-LSTM  b) Ablation qualitative study on Individual MX-LSTM (better in color).}\label{fig:Qualitative}
		\vspace{-15pt}
	\end{center}
    \end{figure*}

\figref{fig:Qualitative} shows  qualitative results on the Zara02 dataset, which was found as the most difficult throughout the quantitative experiments.
%\footnote{Please check supplemental material for further results.}. 
%
\figref{fig:Qualitative}a presents MX-LSTM results: a group scenario is taken into account, with the attention focused on the girl in the bottom-left corner. In the left column, the green ground-truth prediction vislets show that the girl is conversing with the group members, with a movement close to zero and the pan head angle which oscillates. In magenta, the behavior of the S-LSTM, predicting erroneously the girl leaving the group. This error confirms the problem of competing methods in forecasting the motion of people slowly moving or static as discussed in Sec.~\ref{sec:motivation}, and further confirmed by the results of the quantitative experiments. %, which show that when people are moving slowly or are static, forecasting error are in general dramatic.
In the central column, the observation sequence given to the MX-LSTM is shown in orange (almost static with oscillating vislets). The related prediction (in yellow) shows oscillating vislets, and almost no movement, confirming that the MX-LSTM has learnt this particular social behavior. If we provide the MX-LSTM with an artificial observation sequence with the annotated positions (real trajectory) but vislets oriented toward west  (third column, orange arrows), where no people are present, the MX-LSTM predicts a trajectory departing from the group (cyan trajectory and arrows).


The two rows of \figref{fig:Qualitative}b analyze the Individual MX-LSTM, in which no social pooling is taken into account. Here pedestrians are not influenced by the surrounding people, and the forecast motion is only caused by the relationship between the tracklets and the vislets. 
%These figures show different types of trajectories, each one equipped with its own vislets, here represented by the tip of the arrows: the blue one, which represents the routing input sequence given to the MX-LSTM. The green one is the ground-truth that has to be predicted. The yellow one is the prediction by MX-LSTM. The magenta one (left column) has been obtained by enforcing the vislets of the routing input sequence to point north (w.r.t. the image plane). The black one (center column) is the same as the magenta one, but pointing north. The red one (right column) has randomly placed vislets. The rationale of these last three types of sequences is to evaluate whether a different head pose behavior could trigger a diverse trajectory prediction. 
The first row in \figref{fig:Qualitative}b shows three situations in which the vislets of the observation sequence are manually altered to point north (orange arrows), thus orthogonal to the person trajectory. In this case the Individual MX-LSTM predicts a decelerating trajectory drifting toward north (magenta trajectory and vislets), especially visible in the second and third pictures.  If the observation has the legit vislets (green arrows, barely visible since they are aligned with the trajectory), the resulting trajectory (yellow trajectory and vislets) has a different behavior, closer to the GT (green trajectory and vislets). Similarly, in the second row, we altered vislets to point to South. The prediction with the modified vislets is in black. The only difference is in the bottom left picture: here the observation vislets pointing south are in agreement with the movement, so that the resulting predicted trajectory is not decelerating as in the other cases, but accelerating toward south.



%(first column) and south (second column) do have a role in the trajectory prediction, being the related trajectories drifting themselves toward north and south. Interestingly, there is a general deceleration: this is the type of dynamics that happens when a person, while walking, turn his head to an object of interest, and changes direction slowing down to better look at it. Notably, all the vislets points have a distance which is somewhat constant (similar to $r$): this indicates that the LSTM has also captured the (artificial) distance between tracklet and vislet points. The unlikely vislet sequence (the red one, right column) lets the system predicts a fast trajectory with the vislets diverging from the trajectory. 

%\figref{fig:Qualitative} second row
%30 1351  
%shows a %
%-->211359 - 563047
%similar behavior, going left to right: the purple sequence decelerate a little and goes north, the black one goes south.  

%\figref{fig:Qualitative} third row 
%211239 
%shows that, for the individual going south, enforcing the head pose look north slows down dramatically the sequence, while looking south let the individual continue to go in that direction, while the correct trajectory was drifting left.




%%5935 4063 5215

\renewcommand{\arraystretch}{2}
\begin{table}[!b]
  \centering
  \caption{MAD errors on the different datasets including the requested (in bold) MX-LSTM-HPE \emph{Train and Test} and \emph{pace} MX-LSTM}
  \label{table:step}
  \resizebox{.999\linewidth}{!}{\begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Dataset}    & \textbf{MX-LSTM}  & \textbf{\begin{tabular}[c]{@{}c@{}}MX-LSTM-HPE\vspace{-7pt}\\ \textit{Train and Test}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\textit{pace}\vspace{-7pt}\\ \textit{MX-LSTM}\end{tabular}}\\ \hline
    \textbf{Zara01}     &  0.59   &  0.68       &    0.69      \\ \hline
    \textbf{Zara02}     &  0.35   &  0.51     &    0.73            \\ \hline
    \textbf{UCY}        &  0.49   &  0.58               &    0.59          \\ \hline
    \textbf{Town Centre} & 1.15   &  1.43               & 1.50                \\ \hline
  \end{tabular}}
\end{table}
\renewcommand{\arraystretch}{1}



\vspace{-0.2cm}


\vspace{-0.1cm}
    \begin{figure*}[t!] 
	\begin{center}
		\includegraphics[width=1\linewidth]{figure/VFOA.png}
		\caption{VFOA pooling: For a given subject, he will try to avoid collision with the people who are inside his view frustum (blue circle). Others (red circle), will not influence his trajectory as they are no in his view frustum. }\label{fig:vfoaPoolingIllustration}
		\vspace{-15pt}
	\end{center}
    \end{figure*}

% \fs{Please change this picture: first of all, it is hard to convince somebody that the person on the mid left is outside the view frustum of the target individual; second, the yellow arcs are very short, it seems we only take into account very close people. Moreover I would say old frustums are not important here, since the social pooling has no memory. Lastly, it is too big.}









% \iffalse
% \begin{table*}[t]
%   \centering
%   \vspace{10em}
%   \caption{MAD -- Complete table: filled by Irtiza}
%   \label{xx-}
%   \scalebox{.88}{
%   \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
%     \hline
%     Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
%     \hline
%     Zara01    &2.74  &2.88  &0.90  &0.89  &0.58  &0.63  &0.68  &0.66  &0.69 &0.63 &0.60 &0.60 \\
%     \hline
%     Zara02    &2.23  &2.32  &1.1  &0.89  &1.2  &0.72  &0.63  &0.48  &0.43 &0.36 &0.41 &0.35  \\
%     \hline
%     UCY        &2.49  &2.57  &0.67  &0.54  &0.84  &0.53  &0.62  &0.60  &0.58 &0.51 &0.54 &0.49  \\
%     \hline
%     TownCentre &  &  &4.62  &1.96  &2.67  &2.09  &1.96  &1.7  &1.9 &1.7 &1.4 &1.15  \\
%     \hline \hline
%     TownCentre (real HPE) &--  & --  &--  &2.08  &--  &2.18  &--  &1.7  &-- &1.7 &1.44 &1.2  \\
%     \hline
%   \end{tabular}
%   }
%   \caption{FAD -- Complete table: filled by Irtiza}
%   \label{xx-}
%   \scalebox{.88}{
%   \begin{tabular}{|l|*{12}{C{.05\textwidth}|}}
%     \hline
%     Dataset    &  LTA  &  SF   &  LSTM  & Vislet-LSTM & LogCh-LSTM &  LogCh-Vislet-LSTM  &  Social LSTM   &  Social Vislet LSTM  & LogCh-Social LSTM & LogCh-Social Vislet LSTM & Viewfrsutum Social Vislet LSTM & LogCh Viewfrsutum Social Vislet LSTM \\
%     \hline
%     Zara01    &5.55  &5.55  &1.85  &1.81  &1.28  &1.37  &1.53  &1.51  &1.5 &1.40 &1.51 &1.31  \\
%     \hline
%     Zara02    &4.35  &4.35  &2.15  &1.90  &2.69  &1.56  &1.43  &1.06  &1.0 &0.84 &1.00 &0.79  \\
%     \hline
%     UCY        &4.66  &4.62  &1.39  &1.15  &1.92  &1.16  &1.40  &1.36  &1.27 &1.15 &1.23 &1.12  \\
%     \hline
%     TownCentre &  &  &8.26  &3.96  &5.15  &4.0  &3.96  &3.6  &4.2 &3.4 &2.9 &2.3  \\
%     \hline \hline
%     TownCentre (real HPE) &--  &--  &--  &4.12  &--  &4.2  &--  &3.6  &-- &3.4 &3.0 &2.36  \\
%     \hline
%   \end{tabular}
%   }
% \end{table*}







% \fs{TO DO:
% \begin{itemize}
%     \item show the qualitative sequences in the text and show the distributions of LSTM, vislet LSTM (original data) and the distribution of the vislets
%     \item 
% \end{itemize}}
% \fi


==> sections/suppmaterial_text.tex <==

This supplementary material provides additional qualitative results, more details on some of the paper equations, more information on the adopted code and errata to the paper.

Please watch the attached {\tt supmat.mp4} for more qualitative results. In particular, the video illustrates the the role that vislets play in the MX-LSTM.

Additionally, this pdf provides the following:
%In this supplementary material we provide new qualitative results, details omitted in the main text, and we fix a sentence which may rise misunderstandings.
\begin{itemize}
    %\item The video file {\tt xxx.avi} gives qualitative results in addition to those reported in the paper;
    \item Sec.~\ref{sec:ablation} gives the equations for the ablation models;
    \item Sec.~\ref{sec:implementation} details the implementation of the MX-LSTM;
    \item Sec.~\ref{sec:code} provides the http addresses of the code used for the comparative experiments;
    \item Sec.~\ref{sec:errata} revises a sentence in the paper, expressing it in a clearer way.
\end{itemize}

\section{Ablation study: equations}\label{sec:ablation}
On rows 623-630 we introduced the \textbf{Block-Diagonal MX-LSTM (BD-MX-LSTM)}: The equations that differ w.r.t. MX-LSTM's Eq. (7) and (9) are, respectively, 
\begin{eqnarray}
L^i(\mathbf{W}_{x},\mathbf{W}_{a},\mathbf{W}_H,\mathbf{W}_{\text{LSTM}},\mathbf{W}_{o}) &=&\nonumber\\  -\sum_{T_{obs}+1}^{T_{pred}}log\left( P([\mathbf{x}^{(i)}_t]^T|\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t \right)+\!\!\\\nonumber
log\left(P([\mathbf{a}^{(i)}_t]^T|\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t\right)
\end{eqnarray}
where $\bo{\mu}^{(x,i)}_t=[{}_x\mu^{(x,i)}_t,{}_y\mu^{(x,i)}_t]$ and ${}_x\mu^{(x,i)}_t$ is the x-component of $\bo{\mu}$ and the same applies for the standard deviation vector $\bo{\sigma}^{(x,i)}_t$.

The second log term of (1) represents the likelihood's fit for the anchor points of the vislets.
Equation (9) in the main paper becomes:
\begin{equation}
[\bo{\mu}^{(x,i)}_t,\bo{\sigma}^{(x,i)}_t,\rho^{(x,i)}_t,\bo{\mu}^{(a,i)}_t,\bo{\sigma}^{(a,i)}_t,\rho^{(a,i)}_t]^T \!=\! \mathbf{W}_o \mathbf{h}^{(i)}_{t-1}\label{eq:params}
\end{equation}
 
\section{Implementation details} \label{sec:implementation}

For training MX-LSTM and the ablation study models, we use a learning rate of 0.005 along with the RMS-prop optimizer. We set the embedding dimension for spatial coordinates and vislets to 64 and the hidden state dimension is $D=128$.
We plan to release the code upon acceptance. 


\section{Code used for the experiments} \label{sec:code}
\begin{itemize}
    \item Social Force Model (SF)~\cite{yamaguchi2011cvpr}: code received from the authors (in particular, {\tt kyamagu@vision.is.tohoku.ac.jp}) 
    \item Linear Trajectory Avoidance (LTA)~\cite{pellegrini2009iccv}: code received by {\tt kyamagu@vision.is.tohoku.ac.jp}
    \item Vanilla LSTM and Social LSTM (S-LSTM)~\cite{alahi2016cvpr} \url{https://web.stanford.edu/~alahi/index.html#code} 
\end{itemize}


\section{Errata} \label{sec:errata}

Starting from row 742:

``If we provide to MX-LSTM an artificial observation sequence with \textbf{no 
trajectory} but vislets oriented toward west (third column, orange 
arrows), where no people are present, the MX-LSTM predicts a trajectory 
departing from the group (cyan trajectory and arrows).''\\

The sentence above should instead have read:\\

``If we provide to MX-LSTM an artificial observation sequence with \textbf{the annotated positions (\ie the real trajectory)} but vislets oriented toward west (third column, orange arrows), where no people are present, the MX-LSTM predicts a 
trajectory departing from the group (cyan trajectory and arrows).''\\

%%% Fabio's version:
%``If we provide MX-LSTM with a fictitious observation sequence with the real positions (\ie the real trajectory) but vislets oriented toward west (third column, orange arrows), pointing to an opposite direction from the group of people, the MX-LSTM predicts a trajectory departing from the group (cyan trajectory and arrows).''\\

%The misplaced original sentence was due to the fact that the GT trajectory was essentially a point, since the pedestrian is static.

